Efficient Incremental Code Coverage Analysis for Regression Test Suites

Code coverage analysis has been widely adopted in the continuous integration of open-source and industry software repositories to monitor the adequacy of regression test suites. However, computing code coverage can be costly, introducing significant overhead during test execution. Plus, re-collecting code coverage for the entire test suite is usually unnecessary when only a part of the coverage data is affected by code changes. While regression test selection (RTS) techniques exist to select a subset of tests whose behaviors may be affected by code changes, they are not compatible with code coverage analysis techniques -- that is, simply executing RTS-selected tests leads to incorrect code coverage results. In this paper, we present the first incremental code coverage analysis technique, which speeds up code coverage analysis by executing a minimal subset of tests to update the coverage data affected by code changes. We implement our technique in a tool dubbed iJaCoCo, which builds on Ekstazi and JaCoCo -- the state-of-the-art RTS and code coverage analysis tools for Java. We evaluate iJaCoCo on 1,122 versions from 22 open-source repositories and show that iJaCoCo can speed up code coverage analysis time by an average of 1.86x and up to 8.20x compared to JaCoCo.

==> defs/defs-code.tex <==
%%% defs-code.tex
%%% Utility Commands for Code Listings
%%% Version 1.0.2

%%%==========
%%% COPIED FROM vkuncak/doc/vmcai09/defs.tex
\definecolor{gray}{RGB}{211,211,211}
\newcommand{\jbasicstyle}{\small\sffamily} % Style of code
\newcommand{\textcode}[1]{{#1}}
\newcommand{\jnumberstyle}{\scriptsize}
\newcommand{\Hilight}{\makebox[0pt][l]{\color{gray}\rule[-3pt]{0.80\linewidth}{9pt}}}

\lstdefinelanguage{pseudo}
{
  morekeywords={},
  keywordstyle=\bfseries,
  lineskip=-0.1em,
  numbers=left, % none for no numbers
  numberstyle=\jnumberstyle,
  numbersep=4pt,
  basicstyle=\jbasicstyle,
  breaklines=true,
  breakautoindent=true,
  tabsize=2,
  columns=fullflexible,
  morecomment=*[l][\textsl]{//},
  mathescape=true,
  xleftmargin=10pt,
%  mathescape=false,
}

\lstdefinelanguage{todo-comment}
{
  morekeywords={},
  keywordstyle=\bfseries,
  lineskip=-0.1em,
  numbers=none,
  basicstyle=\jbasicstyle,
  breaklines=true,
  breakautoindent=true,
  tabsize=2,
  columns=fullflexible,
  morecomment=*[l][\textsl]{//},
  mathescape=true,
  xleftmargin=-10pt,
%  mathescape=false,
}

\lstdefinelanguage{java-pretty}
{
  language=java,
  numbers=left,
  basicstyle=\scriptsize\ttfamily,
  numberstyle=\scriptsize,
  breaklines=true,
  columns=fullflexible,
  xleftmargin=16pt,
  showstringspaces=false,
}

\lstdefinelanguage{java-pretty-no-number}
{
  language=java,
  numbers=none,
  basicstyle=\scriptsize\ttfamily,
  numberstyle=\scriptsize,
  breaklines=true,
  columns=fullflexible,
  xleftmargin=16pt,
  showstringspaces=false,
}

\lstset{escapeinside={(*@}{@*)}}

%%%==========


==> defs/defs-logic.tex <==
%%% defs-logic.tex
%%% Utility Commands for Logic Symbols
%%% Version 1.1.0

%%% Basic Logic
% True & False
\newcommand{\ltrue}{\top} % ⊤
\newcommand{\lfalse}{\bot} % ⊥

% Operators
% \land ∧
% \lor ∨
% \lnot ¬
\newcommand{\limply}{\rightarrow} % →
\newcommand{\liff}{\leftrightarrow} % ↔
\newcommand{\lcofactor}{\downarrow} % ↓

\newcommand{\llimply}{\Rightarrow} % ⇒
\newcommand{\lliff}{\Leftrightarrow} % ⇔
\newcommand{\lsat}{\vDash} % ⊨
\newcommand{\lnsat}{\nvDash} % ⊭

% Quantifiers
\newcommand{\lqall}[1]{\forall #1.~} % ∀x.
\newcommand{\lqexist}[1]{\exists #1.~} % ∃x.
\newcommand{\lqallOnly}[1]{\forall #1 } % ∀x
\newcommand{\lqexistOnly}[1]{\exists #1 } % ∃x

% Big Operators
\newcommand{\lAnd}[1]{\bigwedge_{\substack{#1}}} % ⋀
\newcommand{\lOr}[1]{\bigvee_{\substack{#1}}} % ⋁

%%% Set
\newcommand{\set}[1]{\{#1\}} % {x, y, z}
\newcommand{\Set}[1]{\left\{#1\right\}} % \left{ x, y, z \right}
\newcommand{\tuple}[1]{\langle#1\rangle} % <a, b, c>
\newcommand{\Tuple}[1]{\left\langle#1\right\rangle} % \left< a, b, c \right>

\newcommand{\sunion}{\cup} % ∪
\newcommand{\sinter}{\cap} % ∩


==> figs/examples/commons-lang_9fb4f47f.tex <==
% | version   |   cov_b |   cov_i |   num_b |   num_i |   num_e |   time_b |   time_i |   speedup_i |   rate_i | diff                                                               |
% | 9fb4f47f  |    0.95 |    0.95 |  149.00 |    4.00 |    4.00 |    29.75 |    18.65 |        1.60 |     0.03 | https://github.com/apache/commons-lang/compare/b1deb442...9fb4f47f |

% old coverage: i 705/718, l 141/144, b 72/80
% new coverage: i 705/716, l 141/143, b 72/80

% |T_rts| = |T_sel| = 4
% org.apache.commons.lang3.builder.ReflectionDiffBuilderTest
% org.apache.commons.lang3.reflect.FieldUtilsTest
% org.apache.commons.lang3.reflect.TypeUtilsTest
% org.apache.commons.lang3.time.StopWatchTest

\newsavebox\boxExampleI
\begin{lrbox}{\boxExampleI}
\begin{lstlisting}[language=java-pretty-no-number]
// org/apache/commons/lang3/reflect/FieldUtils.java
public static void removeFinalModifier(final Field field, 
    final boolean forceAccess) {
  Validate.isTrue(field != null, "The field must not be null");
  try { ...
  } catch (final NoSuchFieldException ignored) {
  } catch (final NoSuchFieldException | IllegalAccessException ignored) {
    // The field class contains always a modifiers field
  } catch (final IllegalAccessException ignored) {
    // The modifiers field is made accessible
  }
}
\end{lstlisting}
\end{lrbox}

\DefMacro*{h-line}{2.16ex}
\DefMacro*{w-line}{27em}

\begin{minipage}{.9\columnwidth}
\begin{tikzpicture}[
    git-add/.style={minimum height=\UseMacro{h-line}, minimum width=\UseMacro{w-line}, text width=\UseMacro{w-line}, text height=0.3 * \UseMacro{h-line}, font=\scriptsize\ttfamily, fill=green!20},
    git-del/.style={minimum height=\UseMacro{h-line}, minimum width=\UseMacro{w-line}, text width=\UseMacro{w-line}, text height=0.3 * \UseMacro{h-line}, font=\scriptsize\ttfamily, fill=red!20},
]{
\coordinate (c-nw) at (0, 0) {};
\node (b-del-6) [below right = 6 * \UseMacro{h-line} and 0 of c-nw] [git-del] {-};
\node (b-add-7) [below right = 7 * \UseMacro{h-line} and 0 of c-nw] [git-add] {+};
\node (b-del-9) [below right = 9.2 * \UseMacro{h-line} and 0 of c-nw] [git-del] {-};
\node (b-del-10) [below right = 10.2 * \UseMacro{h-line} and 0 of c-nw] [git-del] {-};
\node (b-code) [below right = 0 and 0 of c-nw] {\usebox{\boxExampleI}};
}
\end{tikzpicture}
\vspace{-15pt}
\subcaption{Code change between \revision \UseMacro{example1-version-old} and \UseMacro{example1-version-new}. \label{fig:example1:diff}}
\end{minipage}
\\
\begin{minipage}{.9\columnwidth}
\vspace{5pt}
\begin{lstlisting}[language=java-pretty-no-number, frame=single, xleftmargin=2pt, xrightmargin=4em]
org.apache.commons.lang3.builder.ReflectionDiffBuilderTest
org.apache.commons.lang3.reflect.FieldUtilsTest
org.apache.commons.lang3.reflect.TypeUtilsTest
org.apache.commons.lang3.time.StopWatchTest
\end{lstlisting}
\vspace{-3pt}
\subcaption{\Tests selected by \ijacocoTool. \label{fig:example1:tests-ijacoco}}
\end{minipage}


% \includegraphics[width=0.4\columnwidth]{figs/examples/commons-lang_9fb4f47f_coverage_old.png}
% \includegraphics[width=0.4\columnwidth]{figs/examples/commons-lang_9fb4f47f_coverage_new.png}


==> figs/selection-counter-example.tex <==
\newsavebox{\lstExampleSi}
\begin{lrbox}{\lstExampleSi}
\begin{lstlisting}[language=java-pretty, numbersep=2pt]
class c1 {
  c1() {}
  void m() {return;}
}
\end{lstlisting}
\end{lrbox}

\newsavebox{\lstExampleSii}
\begin{lrbox}{\lstExampleSii}
\begin{lstlisting}[language=java-pretty, numbersep=2pt]
class c2 {
  c2() {}
  void m() {new c1().m();}
}
\end{lstlisting}
\end{lrbox}

\newsavebox{\lstExampleSiii}
\begin{lrbox}{\lstExampleSiii}
\begin{lstlisting}[language=java-pretty, numbersep=2pt]
class c3 {
  c3() {}
  void m() {return;}
}
\end{lstlisting}
\end{lrbox}

\newsavebox{\lstExampleTi}
\begin{lrbox}{\lstExampleTi}
\begin{lstlisting}[language=java-pretty, numbersep=2pt]
class t1 {
  @Test void t() {
    new c1();
}}
\end{lstlisting}
\end{lrbox}

\newsavebox{\lstExampleTii}
\begin{lrbox}{\lstExampleTii}
\begin{lstlisting}[language=java-pretty, numbersep=2pt]
class t2 {
  @Test void t() {
    new c2().m();
}}
\end{lstlisting}
\end{lrbox}

\newsavebox{\lstExampleTiii}
\begin{lrbox}{\lstExampleTiii}
\begin{lstlisting}[language=java-pretty, numbersep=2pt]
class t3 {
  @Test void t() {
    new c3();
}}
\end{lstlisting}
\end{lrbox}


\DefMacro*{xsep}{3em}
\DefMacro*{ysep}{2ex}

\begin{tikzpicture}[
  font=\footnotesize, 
  codeblock/.style={rectangle, rounded corners, draw=black, minimum height=4ex, inner xsep=8pt},
  test codeblock/.style={codeblock, text width=6em},
  src codeblock/.style={codeblock, text width=9em},
  anno/.style={font={\footnotesize}},
]

\coordinate (c-0) at (0, 0);

\coordinate (c-test) at (c-0);
\node (b-t1) [below right = 0 and 0 of c-test, anchor=north west]
[test codeblock] 
{\usebox{\lstExampleTi}};

\node (b-t2) [below right = \UseMacro{ysep} and 0 of b-t1.south west, anchor=north west]
[test codeblock] 
{\usebox{\lstExampleTii}};

\node (b-t3) [below right = \UseMacro{ysep} and 0 of b-t2.south west, anchor=north west]
[test codeblock] 
{\usebox{\lstExampleTiii}};

\coordinate (c-src) at ($(c-test -| b-t1.east) + (\UseMacro{xsep}, 0)$);
\node (b-c1) [below right = 0 and 0 of c-src, anchor=north west]
[src codeblock] 
{\usebox{\lstExampleSi}};

\node (b-c2) [below right = \UseMacro{ysep} and 0 of b-c1.south west, anchor=north west]
[src codeblock] 
{\usebox{\lstExampleSii}};

\coordinate (c-diffs) at ($(b-c2.east) + (0, -2ex)$);
\node (b-diff1) [above right = 0.5ex and 1em of c-diffs]
[anno]
{\circled{a} \CodeIn{return;}};
\node (b-diff2) [below right = 0.5ex and 1em of c-diffs]
[anno]
{\circled{b} \CodeIn{new\ c3().m();}};
\node (anno-diffs) [above = 0.5ex of b-diff1.north]
[anno]
{\emph{possible \changeset}};

\node (b-c3) [below right = \UseMacro{ysep} and 0 of b-c2.south west, anchor=north west]
[src codeblock] 
{\usebox{\lstExampleSiii}};

\draw[->] (b-t1) -- (b-c1);
\draw[->] (b-t2) -- (b-c2);
\draw[->] (b-t3) -- (b-c3);
\draw[->] (b-c2) -- (b-c1);

\draw[dotted, thick] (c-diffs) -- (b-diff1.west);
\draw[dotted, thick] (c-diffs) -- (b-diff2.west);

\end{tikzpicture}


==> figs/workflow.tex <==
\DefMacro*{x-phase}{8em}
\DefMacro*{xsep-phase}{2em}
\DefMacro*{ysep-phase}{2ex}

\begin{tikzpicture}[
  font=\small, 
  box/.style={rectangle, scale=1, inner sep=1pt, rounded corners=5pt, thick},
  label/.style={scale=0.9, font={\bfseries\sc}},
  anno/.style={font={\footnotesize}},
]

\coordinate (c-0) at (0,0) {};

% phases
\node (b-analysis) at (c-0)
[box, minimum width=14em, minimum height=30ex] 
[draw=blue!50!black, fill=blue!10]
{};
\node (l-analysis) [below left = 0 and 0 of b-analysis.north east] [label] {\Analysis};

\node (b-execution) [below right = 2ex and \UseMacro{xsep-phase} of b-analysis.north east] 
[box, minimum width=\UseMacro{x-phase}, minimum height=6ex] 
[draw=red!50!black, fill=red!10]
{};
\node (l-execution) [below left = 0 and 0 of b-execution.north east] [label] {\Execution};

\node (b-collection) [below = \UseMacro{ysep-phase} of b-execution] 
[box, minimum width=\UseMacro{x-phase}, minimum height=16ex] 
[draw=yellow!50!black, fill=yellow!10]
{};
\node (l-collection) [below left = 0 and 0 of b-collection.north east] [label] {\Collection};

% \node (b-report) [below = \UseMacro{ysep-phase} of b-collection] 
% [box, minimum width=\UseMacro{x-phase}, minimum height=9ex] 
% [draw=green!50!black, fill=green!10]
% {};
% \node (l-report) [below left = 0 and 0 of b-report.north east] [label] {\Report};

% analysis inputs
\coordinate (cy-tests) at (b-execution);
\coordinate (cy-dependency) at ($(b-collection.north) + (0, -4ex)$);
\coordinate (cy-covdata) at ($(b-collection.south) + (0, 4ex)$);
% \coordinate (cy-report) at ($(b-report.north) + (0, -4ex)$);

\coordinate (cx-input) at ($(b-analysis.west) + (2em, 0)$);

\coordinate (c-ClassSetChanged) at (cx-input |- cy-tests);
\node (l-ClassSetChanged) at (c-ClassSetChanged)
[anno]
{\aClassSetChanged};
\node (anno-ClassSetChanged) [below left = -0.5ex and 1em of l-ClassSetChanged.south west, anchor=north west]
[anno]
{change set};

\coordinate (c-DepGraphOld) at (cx-input |- cy-dependency);
\node (l-DepGraphOld) at (c-DepGraphOld)
[anno]
{\aDepGraphOld};
\node (anno-DepGraphOld) [below left = -0.5ex and 1em of l-DepGraphOld.south west, anchor=north west]
[anno]
{dependency graph};

\coordinate (c-CovDataOld) at (cx-input |- cy-covdata);
\node (l-CovDataOld) at (c-CovDataOld)
[anno]
{\aCovDataOld};
\node (anno-CovDataOld) [below left = -0.5ex and 1em of l-CovDataOld.south west, anchor=north west]
[anno]
{\covdata};

% analysis steps
\coordinate (cx-analysis1) at ($(b-analysis.west)!0.35!(b-analysis.east)$);
\coordinate (cx-analysis2) at ($(b-analysis.west)!0.6!(b-analysis.east)$);
\coordinate (cx-analysis3) at ($(cx-analysis2) + (1.65em, 0)$);
\coordinate (cx-analysis4) at ($(b-analysis.west)!0.875!(b-analysis.east)$);

\coordinate (c-TestSetNewSelectedRTS) at (cx-analysis1 |- cy-tests);
\node (l-TestSetNewSelectedRTS) at (c-TestSetNewSelectedRTS)
[anno]
{\aTestSetNewSelectedRTS};

\coordinate (cy-tests-collection) at ($(b-execution)!0.5!(b-collection)$);
\coordinate (c-ClassSetCovInvalid) at (cx-analysis2 |- cy-tests-collection);
\node (l-ClassSetCovInvalid) at (c-ClassSetCovInvalid)
[anno]
{\aClassSetCovInvalid};

\node (l-RemoveCovData) at (cx-analysis3 |- cy-covdata)
[anno, scale=1.5, inner sep=0]
{$\ominus$};
\node (anno-RemoveCovData) [below = -0.5ex of l-RemoveCovData.south]
[anno]
{remove outdated};

\coordinate (c-TestSetNewSelectedI) at (cx-analysis4 |- cy-tests);
\node (l-TestSetNewSelectedI) at (c-TestSetNewSelectedI)
[anno]
{\aTestSetNewSelectedI};

% execution, collection steps
\coordinate (cx-covdata-joint) at ($(b-collection.west)!0.15!(b-collection.east)$);
\coordinate (cx-collection-joint) at ($(cx-covdata-joint) + (1.5em, 0)$);
\coordinate (cx-collection-output) at ($(b-collection.west)!0.55!(b-collection.east)$);
\coordinate (cx-covdata-output1) at ($(b-collection.west)!0.55!(b-collection.east)$);
\coordinate (cx-covdata-output2) at ($(b-collection.west)!0.85!(b-collection.east)$);
\coordinate (cy-covdata-output2) at ($(cy-covdata)!0.6!(b-collection.south)$);

\node (l-CovDataDiff) at (cx-covdata-joint |- cy-tests)
[anno]
{\aCovDataDiff};

\node (l-DepGraphDiff) at (cx-collection-joint |- cy-tests)
[anno]
{\aDepGraphDiff};

\node (l-DepGraphNew) at (cx-collection-output |- cy-dependency)
[anno]
{\aDepGraphNew};

\node (l-CovDataNew) at (cx-covdata-output1 |- cy-covdata)
[anno]
{\aCovDataNew};

% \node (l-ElemSetCoveredNew) at (cx-covdata-output2 |- cy-covdata-output2)
% [anno]
% {\makecell[c]{\aElemSetCoveredNew\\\aCoverage}};

\node (l-ReportGen) at (cx-covdata-output1 |- b-analysis.south)
[anno, yshift=1ex]
{report generation};

\node (l-MergeDepGraph) at (cx-collection-joint |- cy-dependency)
[anno, scale=1.5, inner sep=0]
{$\oplus$};
\node (anno-MergeDepGraph) [below = -0.5ex of l-MergeDepGraph.south]
[anno]
{merge};

\node (l-MergeCovData) at (cx-covdata-joint |- cy-covdata)
[anno, scale=1.5, inner sep=0]
{$\oplus$};
\node (anno-MergeCovData) [below = -0.5ex of l-MergeCovData.south]
[anno]
{merge};

% in/out
\coordinate (cx-lastv) at ($(b-analysis.west) + (-0.5em, 0)$);
\coordinate (cx-nextv) at ($(b-collection.east) + (0.5em, 0)$);
\coordinate (cy-dependency-covdata) at ($(cy-dependency)!0.5!(cy-covdata)$);

\node (l-lastv) at (cx-lastv |- cy-dependency-covdata)
[anno, rotate=270, yshift=-1em]
{from old \revision};
\node (l-nextv) at (cx-nextv |- cy-dependency-covdata)
[anno, rotate=270, yshift=1em]
{to next \revision};

% wire everything together
\draw[->] (l-ClassSetChanged) -- (l-TestSetNewSelectedRTS);
\draw[->] (l-TestSetNewSelectedRTS) -- (l-TestSetNewSelectedI);
\draw[->] (l-TestSetNewSelectedI) -- (b-execution.west);
\draw[->] (l-DepGraphOld) -- (l-MergeDepGraph);
\draw[->] (l-MergeDepGraph) -- (l-DepGraphNew);
\draw[->] (l-CovDataOld) -- (l-RemoveCovData);
\draw[->] (l-RemoveCovData) -- (l-MergeCovData);
\draw[->] (l-MergeCovData) -- (l-CovDataNew);
\draw[->] (cx-lastv |- l-DepGraphOld) -- (l-DepGraphOld);
\draw[->] (cx-lastv |- l-CovDataOld) -- (l-CovDataOld);
\draw[->] (l-DepGraphNew) -- (cx-nextv |- l-DepGraphNew);
\draw[->] (l-CovDataNew) -- (cx-nextv |- l-CovDataNew);
\draw[->] (l-CovDataDiff) -- (l-MergeCovData);
\draw[->] (l-DepGraphDiff) -- (l-MergeDepGraph);

\draw[->, rounded corners=3pt] (l-DepGraphOld.east) -- ($(l-DepGraphOld.east) + (1em, 0)$) -- ($(l-ClassSetCovInvalid.west) + (-0.5em, 0)$) -- (l-ClassSetCovInvalid.west);
\draw[rounded corners=3pt] (l-TestSetNewSelectedRTS.east) -- ($(l-TestSetNewSelectedRTS.east) + (0.5em, 0)$) -- ($(l-ClassSetCovInvalid.west) + (-0.5em, 0)$) -- (l-ClassSetCovInvalid.west);

\draw[rounded corners=3pt] (l-ClassSetCovInvalid.east) -- ($(l-ClassSetCovInvalid.east) + (0.5em, 0)$) -- ($(l-TestSetNewSelectedI.west) + (-1em, 0)$) -- (l-TestSetNewSelectedI.west);

% \draw[->, rounded corners=3pt] (l-CovDataNew.east) -- ($(l-CovDataNew.east) + (0.5em, 0)$) -- ($(l-ElemSetCoveredNew.west) + (-0.5em, 0)$) -- (l-ElemSetCoveredNew.west);

\draw[->] (l-CovDataNew.south) -- (l-ReportGen.north);

\draw[->, rounded corners=3pt] (l-ClassSetCovInvalid.east) -| (l-RemoveCovData.north);

\end{tikzpicture}

==> tables/table-projects.tex <==
%% Automatically generated by: results.py table_projects_results

\begin{tabular}{l|l|c|r|r|r|r|r}
\toprule
\multicolumn{1}{c|}{\multirow{2}{*}{\textbf{\UseMacro{TH-project}}}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{\UseMacro{TH-head-revision}}}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{\UseMacro{TH-num-revision}}}} & \multicolumn{2}{c|}{\textbf{\UseMacro{TH-project-size}}} & \multicolumn{3}{c}{\textbf{\UseMacro{TH-project-test}}} \\
& & & \multicolumn{1}{c}{\UseMacro{TH-num-file}} & \multicolumn{1}{c|}{\UseMacro{TH-loc}} & \multicolumn{1}{c}{\UseMacro{TH-num-test-class}} & \multicolumn{1}{c}{\UseMacro{TH-num-test-method}} & \multicolumn{1}{c}{\UseMacro{TH-test-time}} \\
\midrule
\href{\UseMacro{res-asterisk-java-asterisk-java-url}}{\UseMacro{res-asterisk-java-asterisk-java-name}} & \texttt{\UseMacro{res-asterisk-java-asterisk-java-head}} & \UseMacro{res-asterisk-java-asterisk-java-num-ver} & \UseMacro{res-asterisk-java-asterisk-java-num-file} & \UseMacro{res-asterisk-java-asterisk-java-loc} & \UseMacro{res-asterisk-java-asterisk-java-num-class} & \UseMacro{res-asterisk-java-asterisk-java-num-method} & \UseMacro{res-asterisk-java-asterisk-java-time}    \\
\href{\UseMacro{res-apache-commons-beanutils-url}}{\UseMacro{res-apache-commons-beanutils-name}} & \texttt{\UseMacro{res-apache-commons-beanutils-head}} & \UseMacro{res-apache-commons-beanutils-num-ver} & \UseMacro{res-apache-commons-beanutils-num-file} & \UseMacro{res-apache-commons-beanutils-loc} & \UseMacro{res-apache-commons-beanutils-num-class} & \UseMacro{res-apache-commons-beanutils-num-method} & \UseMacro{res-apache-commons-beanutils-time}    \\
\href{\UseMacro{res-apache-commons-codec-url}}{\UseMacro{res-apache-commons-codec-name}} & \texttt{\UseMacro{res-apache-commons-codec-head}} & \UseMacro{res-apache-commons-codec-num-ver} & \UseMacro{res-apache-commons-codec-num-file} & \UseMacro{res-apache-commons-codec-loc} & \UseMacro{res-apache-commons-codec-num-class} & \UseMacro{res-apache-commons-codec-num-method} & \UseMacro{res-apache-commons-codec-time}    \\
\href{\UseMacro{res-apache-commons-collections-url}}{\UseMacro{res-apache-commons-collections-name}} & \texttt{\UseMacro{res-apache-commons-collections-head}} & \UseMacro{res-apache-commons-collections-num-ver} & \UseMacro{res-apache-commons-collections-num-file} & \UseMacro{res-apache-commons-collections-loc} & \UseMacro{res-apache-commons-collections-num-class} & \UseMacro{res-apache-commons-collections-num-method} & \UseMacro{res-apache-commons-collections-time}    \\
\href{\UseMacro{res-apache-commons-compress-url}}{\UseMacro{res-apache-commons-compress-name}} & \texttt{\UseMacro{res-apache-commons-compress-head}} & \UseMacro{res-apache-commons-compress-num-ver} & \UseMacro{res-apache-commons-compress-num-file} & \UseMacro{res-apache-commons-compress-loc} & \UseMacro{res-apache-commons-compress-num-class} & \UseMacro{res-apache-commons-compress-num-method} & \UseMacro{res-apache-commons-compress-time}    \\
\href{\UseMacro{res-apache-commons-configuration-url}}{\UseMacro{res-apache-commons-configuration-name}} & \texttt{\UseMacro{res-apache-commons-configuration-head}} & \UseMacro{res-apache-commons-configuration-num-ver} & \UseMacro{res-apache-commons-configuration-num-file} & \UseMacro{res-apache-commons-configuration-loc} & \UseMacro{res-apache-commons-configuration-num-class} & \UseMacro{res-apache-commons-configuration-num-method} & \UseMacro{res-apache-commons-configuration-time}    \\
\href{\UseMacro{res-apache-commons-dbcp-url}}{\UseMacro{res-apache-commons-dbcp-name}} & \texttt{\UseMacro{res-apache-commons-dbcp-head}} & \UseMacro{res-apache-commons-dbcp-num-ver} & \UseMacro{res-apache-commons-dbcp-num-file} & \UseMacro{res-apache-commons-dbcp-loc} & \UseMacro{res-apache-commons-dbcp-num-class} & \UseMacro{res-apache-commons-dbcp-num-method} & \UseMacro{res-apache-commons-dbcp-time}    \\
\href{\UseMacro{res-apache-commons-imaging-url}}{\UseMacro{res-apache-commons-imaging-name}} & \texttt{\UseMacro{res-apache-commons-imaging-head}} & \UseMacro{res-apache-commons-imaging-num-ver} & \UseMacro{res-apache-commons-imaging-num-file} & \UseMacro{res-apache-commons-imaging-loc} & \UseMacro{res-apache-commons-imaging-num-class} & \UseMacro{res-apache-commons-imaging-num-method} & \UseMacro{res-apache-commons-imaging-time}    \\
\href{\UseMacro{res-apache-commons-io-url}}{\UseMacro{res-apache-commons-io-name}} & \texttt{\UseMacro{res-apache-commons-io-head}} & \UseMacro{res-apache-commons-io-num-ver} & \UseMacro{res-apache-commons-io-num-file} & \UseMacro{res-apache-commons-io-loc} & \UseMacro{res-apache-commons-io-num-class} & \UseMacro{res-apache-commons-io-num-method} & \UseMacro{res-apache-commons-io-time}    \\
\href{\UseMacro{res-apache-commons-lang-url}}{\UseMacro{res-apache-commons-lang-name}} & \texttt{\UseMacro{res-apache-commons-lang-head}} & \UseMacro{res-apache-commons-lang-num-ver} & \UseMacro{res-apache-commons-lang-num-file} & \UseMacro{res-apache-commons-lang-loc} & \UseMacro{res-apache-commons-lang-num-class} & \UseMacro{res-apache-commons-lang-num-method} & \UseMacro{res-apache-commons-lang-time}    \\
\href{\UseMacro{res-apache-commons-math-url}}{\UseMacro{res-apache-commons-math-name}} & \texttt{\UseMacro{res-apache-commons-math-head}} & \UseMacro{res-apache-commons-math-num-ver} & \UseMacro{res-apache-commons-math-num-file} & \UseMacro{res-apache-commons-math-loc} & \UseMacro{res-apache-commons-math-num-class} & \UseMacro{res-apache-commons-math-num-method} & \UseMacro{res-apache-commons-math-time}    \\
\href{\UseMacro{res-apache-commons-net-url}}{\UseMacro{res-apache-commons-net-name}} & \texttt{\UseMacro{res-apache-commons-net-head}} & \UseMacro{res-apache-commons-net-num-ver} & \UseMacro{res-apache-commons-net-num-file} & \UseMacro{res-apache-commons-net-loc} & \UseMacro{res-apache-commons-net-num-class} & \UseMacro{res-apache-commons-net-num-method} & \UseMacro{res-apache-commons-net-time}    \\
\href{\UseMacro{res-apache-commons-pool-url}}{\UseMacro{res-apache-commons-pool-name}} & \texttt{\UseMacro{res-apache-commons-pool-head}} & \UseMacro{res-apache-commons-pool-num-ver} & \UseMacro{res-apache-commons-pool-num-file} & \UseMacro{res-apache-commons-pool-loc} & \UseMacro{res-apache-commons-pool-num-class} & \UseMacro{res-apache-commons-pool-num-method} & \UseMacro{res-apache-commons-pool-time}    \\
\href{\UseMacro{res-alibaba-fastjson-url}}{\UseMacro{res-alibaba-fastjson-name}} & \texttt{\UseMacro{res-alibaba-fastjson-head}} & \UseMacro{res-alibaba-fastjson-num-ver} & \UseMacro{res-alibaba-fastjson-num-file} & \UseMacro{res-alibaba-fastjson-loc} & \UseMacro{res-alibaba-fastjson-num-class} & \UseMacro{res-alibaba-fastjson-num-method} & \UseMacro{res-alibaba-fastjson-time}    \\
\href{\UseMacro{res-finmath-finmath-lib-url}}{\UseMacro{res-finmath-finmath-lib-name}} & \texttt{\UseMacro{res-finmath-finmath-lib-head}} & \UseMacro{res-finmath-finmath-lib-num-ver} & \UseMacro{res-finmath-finmath-lib-num-file} & \UseMacro{res-finmath-finmath-lib-loc} & \UseMacro{res-finmath-finmath-lib-num-class} & \UseMacro{res-finmath-finmath-lib-num-method} & \UseMacro{res-finmath-finmath-lib-time}    \\
\href{\UseMacro{res-sonyxperiadev-gerrit-events-url}}{\UseMacro{res-sonyxperiadev-gerrit-events-name}} & \texttt{\UseMacro{res-sonyxperiadev-gerrit-events-head}} & \UseMacro{res-sonyxperiadev-gerrit-events-num-ver} & \UseMacro{res-sonyxperiadev-gerrit-events-num-file} & \UseMacro{res-sonyxperiadev-gerrit-events-loc} & \UseMacro{res-sonyxperiadev-gerrit-events-num-class} & \UseMacro{res-sonyxperiadev-gerrit-events-num-method} & \UseMacro{res-sonyxperiadev-gerrit-events-time}    \\
\href{\UseMacro{res-brettwooldridge-HikariCP-url}}{\UseMacro{res-brettwooldridge-HikariCP-name}} & \texttt{\UseMacro{res-brettwooldridge-HikariCP-head}} & \UseMacro{res-brettwooldridge-HikariCP-num-ver} & \UseMacro{res-brettwooldridge-HikariCP-num-file} & \UseMacro{res-brettwooldridge-HikariCP-loc} & \UseMacro{res-brettwooldridge-HikariCP-num-class} & \UseMacro{res-brettwooldridge-HikariCP-num-method} & \UseMacro{res-brettwooldridge-HikariCP-time}    \\
\href{\UseMacro{res-lmdbjava-lmdbjava-url}}{\UseMacro{res-lmdbjava-lmdbjava-name}} & \texttt{\UseMacro{res-lmdbjava-lmdbjava-head}} & \UseMacro{res-lmdbjava-lmdbjava-num-ver} & \UseMacro{res-lmdbjava-lmdbjava-num-file} & \UseMacro{res-lmdbjava-lmdbjava-loc} & \UseMacro{res-lmdbjava-lmdbjava-num-class} & \UseMacro{res-lmdbjava-lmdbjava-num-method} & \UseMacro{res-lmdbjava-lmdbjava-time}    \\
\href{\UseMacro{res-logic-ng-LogicNG-url}}{\UseMacro{res-logic-ng-LogicNG-name}} & \texttt{\UseMacro{res-logic-ng-LogicNG-head}} & \UseMacro{res-logic-ng-LogicNG-num-ver} & \UseMacro{res-logic-ng-LogicNG-num-file} & \UseMacro{res-logic-ng-LogicNG-loc} & \UseMacro{res-logic-ng-LogicNG-num-class} & \UseMacro{res-logic-ng-LogicNG-num-method} & \UseMacro{res-logic-ng-LogicNG-time}    \\
\href{\UseMacro{res-davidmoten-rxjava-extras-url}}{\UseMacro{res-davidmoten-rxjava-extras-name}} & \texttt{\UseMacro{res-davidmoten-rxjava-extras-head}} & \UseMacro{res-davidmoten-rxjava-extras-num-ver} & \UseMacro{res-davidmoten-rxjava-extras-num-file} & \UseMacro{res-davidmoten-rxjava-extras-loc} & \UseMacro{res-davidmoten-rxjava-extras-num-class} & \UseMacro{res-davidmoten-rxjava-extras-num-method} & \UseMacro{res-davidmoten-rxjava-extras-time}    \\
\href{\UseMacro{res-bullhorn-sdk-rest-url}}{\UseMacro{res-bullhorn-sdk-rest-name}} & \texttt{\UseMacro{res-bullhorn-sdk-rest-head}} & \UseMacro{res-bullhorn-sdk-rest-num-ver} & \UseMacro{res-bullhorn-sdk-rest-num-file} & \UseMacro{res-bullhorn-sdk-rest-loc} & \UseMacro{res-bullhorn-sdk-rest-num-class} & \UseMacro{res-bullhorn-sdk-rest-num-method} & \UseMacro{res-bullhorn-sdk-rest-time}    \\
\href{\UseMacro{res-tabulapdf-tabula-java-url}}{\UseMacro{res-tabulapdf-tabula-java-name}} & \texttt{\UseMacro{res-tabulapdf-tabula-java-head}} & \UseMacro{res-tabulapdf-tabula-java-num-ver} & \UseMacro{res-tabulapdf-tabula-java-num-file} & \UseMacro{res-tabulapdf-tabula-java-loc} & \UseMacro{res-tabulapdf-tabula-java-num-class} & \UseMacro{res-tabulapdf-tabula-java-num-method} & \UseMacro{res-tabulapdf-tabula-java-time}    \\
\midrule
\multicolumn{1}{c|}{\UseMacro{TH-sum}} & \UseMacro{TH-na} & \UseMacro{TH-na} & \UseMacro{res-projects-sum-num-file} & \UseMacro{res-projects-sum-loc} & \UseMacro{res-projects-sum-num-test-class} & \UseMacro{res-projects-sum-num-test-method} & \UseMacro{res-projects-sum-time} \\
\bottomrule \end{tabular}

==> tables/table-results-coverage.tex <==
%% Automatically generated by: results.py table_results_coverage

\begin{tabular}{l |r|r|r |r|r|r |r |r|r}
\toprule
\multicolumn{1}{c|}{\multirow{3}{*}{\textbf{\UseMacro{TH-project}}}} & \multicolumn{7}{c|}{\textbf{\UseMacro{TH-coverage}}} & \multicolumn{2}{c}{\textbf{\UseMacro{TH-correctness}}} \\
& \multicolumn{3}{c|}{\bjacoco} & \multicolumn{3}{c|}{\ijacocoTool} &  & \multirow{2}{*}{\UseMacro{TH-exact-same}} & \multirow{2}{*}{\UseMacro{TH-no-stat-sign-diff}}\\
& \UseMacro{TH-min} & \UseMacro{TH-max} & \UseMacro{TH-avg} & \UseMacro{TH-min} & \UseMacro{TH-max} & \UseMacro{TH-avg} & \multicolumn{1}{c|}{\UseMacro{TH-diff}} &  &\\
\midrule
\UseMacro{res-asterisk-java-asterisk-java-name} & \UseMacro{res-asterisk-java-asterisk-java-bjacoco-min-coverage} & \UseMacro{res-asterisk-java-asterisk-java-bjacoco-max-coverage} & \UseMacro{res-asterisk-java-asterisk-java-bjacoco-coverage} & \UseMacro{res-asterisk-java-asterisk-java-ijacoco-min-coverage} & \UseMacro{res-asterisk-java-asterisk-java-ijacoco-max-coverage} & \UseMacro{res-asterisk-java-asterisk-java-ijacoco-coverage} &  \UseMacro{asterisk-java-asterisk-java-coverage-diff} & \UseMacro{asterisk-java-asterisk-java-coverage-exact-same} & \UseMacro{asterisk-java-asterisk-java-coverage-no-stat-sign-diff} \\
\UseMacro{res-apache-commons-beanutils-name} & \UseMacro{res-apache-commons-beanutils-bjacoco-min-coverage} & \UseMacro{res-apache-commons-beanutils-bjacoco-max-coverage} & \UseMacro{res-apache-commons-beanutils-bjacoco-coverage} & \UseMacro{res-apache-commons-beanutils-ijacoco-min-coverage} & \UseMacro{res-apache-commons-beanutils-ijacoco-max-coverage} & \UseMacro{res-apache-commons-beanutils-ijacoco-coverage} &  \UseMacro{apache-commons-beanutils-coverage-diff} & \UseMacro{apache-commons-beanutils-coverage-exact-same} & \UseMacro{apache-commons-beanutils-coverage-no-stat-sign-diff} \\
\UseMacro{res-apache-commons-codec-name} & \UseMacro{res-apache-commons-codec-bjacoco-min-coverage} & \UseMacro{res-apache-commons-codec-bjacoco-max-coverage} & \UseMacro{res-apache-commons-codec-bjacoco-coverage} & \UseMacro{res-apache-commons-codec-ijacoco-min-coverage} & \UseMacro{res-apache-commons-codec-ijacoco-max-coverage} & \UseMacro{res-apache-commons-codec-ijacoco-coverage} &  \UseMacro{apache-commons-codec-coverage-diff} & \UseMacro{apache-commons-codec-coverage-exact-same} & \UseMacro{apache-commons-codec-coverage-no-stat-sign-diff} \\
\UseMacro{res-apache-commons-collections-name} & \UseMacro{res-apache-commons-collections-bjacoco-min-coverage} & \UseMacro{res-apache-commons-collections-bjacoco-max-coverage} & \UseMacro{res-apache-commons-collections-bjacoco-coverage} & \UseMacro{res-apache-commons-collections-ijacoco-min-coverage} & \UseMacro{res-apache-commons-collections-ijacoco-max-coverage} & \UseMacro{res-apache-commons-collections-ijacoco-coverage} &  \UseMacro{apache-commons-collections-coverage-diff} & \UseMacro{apache-commons-collections-coverage-exact-same} & \UseMacro{apache-commons-collections-coverage-no-stat-sign-diff} \\
\UseMacro{res-apache-commons-compress-name} & \UseMacro{res-apache-commons-compress-bjacoco-min-coverage} & \UseMacro{res-apache-commons-compress-bjacoco-max-coverage} & \UseMacro{res-apache-commons-compress-bjacoco-coverage} & \UseMacro{res-apache-commons-compress-ijacoco-min-coverage} & \UseMacro{res-apache-commons-compress-ijacoco-max-coverage} & \UseMacro{res-apache-commons-compress-ijacoco-coverage} &  \UseMacro{apache-commons-compress-coverage-diff} & \UseMacro{apache-commons-compress-coverage-exact-same} & \UseMacro{apache-commons-compress-coverage-no-stat-sign-diff} \\
\UseMacro{res-apache-commons-configuration-name} & \UseMacro{res-apache-commons-configuration-bjacoco-min-coverage} & \UseMacro{res-apache-commons-configuration-bjacoco-max-coverage} & \UseMacro{res-apache-commons-configuration-bjacoco-coverage} & \UseMacro{res-apache-commons-configuration-ijacoco-min-coverage} & \UseMacro{res-apache-commons-configuration-ijacoco-max-coverage} & \UseMacro{res-apache-commons-configuration-ijacoco-coverage} &  \UseMacro{apache-commons-configuration-coverage-diff} & \UseMacro{apache-commons-configuration-coverage-exact-same} & \UseMacro{apache-commons-configuration-coverage-no-stat-sign-diff} \\
\UseMacro{res-apache-commons-dbcp-name} & \UseMacro{res-apache-commons-dbcp-bjacoco-min-coverage} & \UseMacro{res-apache-commons-dbcp-bjacoco-max-coverage} & \UseMacro{res-apache-commons-dbcp-bjacoco-coverage} & \UseMacro{res-apache-commons-dbcp-ijacoco-min-coverage} & \UseMacro{res-apache-commons-dbcp-ijacoco-max-coverage} & \UseMacro{res-apache-commons-dbcp-ijacoco-coverage} &  \UseMacro{apache-commons-dbcp-coverage-diff} & \UseMacro{apache-commons-dbcp-coverage-exact-same} & \UseMacro{apache-commons-dbcp-coverage-no-stat-sign-diff} \\
\UseMacro{res-apache-commons-imaging-name} & \UseMacro{res-apache-commons-imaging-bjacoco-min-coverage} & \UseMacro{res-apache-commons-imaging-bjacoco-max-coverage} & \UseMacro{res-apache-commons-imaging-bjacoco-coverage} & \UseMacro{res-apache-commons-imaging-ijacoco-min-coverage} & \UseMacro{res-apache-commons-imaging-ijacoco-max-coverage} & \UseMacro{res-apache-commons-imaging-ijacoco-coverage} &  \UseMacro{apache-commons-imaging-coverage-diff} & \UseMacro{apache-commons-imaging-coverage-exact-same} & \UseMacro{apache-commons-imaging-coverage-no-stat-sign-diff} \\
\UseMacro{res-apache-commons-io-name} & \UseMacro{res-apache-commons-io-bjacoco-min-coverage} & \UseMacro{res-apache-commons-io-bjacoco-max-coverage} & \UseMacro{res-apache-commons-io-bjacoco-coverage} & \UseMacro{res-apache-commons-io-ijacoco-min-coverage} & \UseMacro{res-apache-commons-io-ijacoco-max-coverage} & \UseMacro{res-apache-commons-io-ijacoco-coverage} &  \UseMacro{apache-commons-io-coverage-diff} & \UseMacro{apache-commons-io-coverage-exact-same} & \UseMacro{apache-commons-io-coverage-no-stat-sign-diff} \\
\UseMacro{res-apache-commons-lang-name} & \UseMacro{res-apache-commons-lang-bjacoco-min-coverage} & \UseMacro{res-apache-commons-lang-bjacoco-max-coverage} & \UseMacro{res-apache-commons-lang-bjacoco-coverage} & \UseMacro{res-apache-commons-lang-ijacoco-min-coverage} & \UseMacro{res-apache-commons-lang-ijacoco-max-coverage} & \UseMacro{res-apache-commons-lang-ijacoco-coverage} &  \UseMacro{apache-commons-lang-coverage-diff} & \UseMacro{apache-commons-lang-coverage-exact-same} & \UseMacro{apache-commons-lang-coverage-no-stat-sign-diff} \\
\UseMacro{res-apache-commons-math-name} & \UseMacro{res-apache-commons-math-bjacoco-min-coverage} & \UseMacro{res-apache-commons-math-bjacoco-max-coverage} & \UseMacro{res-apache-commons-math-bjacoco-coverage} & \UseMacro{res-apache-commons-math-ijacoco-min-coverage} & \UseMacro{res-apache-commons-math-ijacoco-max-coverage} & \UseMacro{res-apache-commons-math-ijacoco-coverage} &  \UseMacro{apache-commons-math-coverage-diff} & \UseMacro{apache-commons-math-coverage-exact-same} & \UseMacro{apache-commons-math-coverage-no-stat-sign-diff} \\
\UseMacro{res-apache-commons-net-name} & \UseMacro{res-apache-commons-net-bjacoco-min-coverage} & \UseMacro{res-apache-commons-net-bjacoco-max-coverage} & \UseMacro{res-apache-commons-net-bjacoco-coverage} & \UseMacro{res-apache-commons-net-ijacoco-min-coverage} & \UseMacro{res-apache-commons-net-ijacoco-max-coverage} & \UseMacro{res-apache-commons-net-ijacoco-coverage} &  \UseMacro{apache-commons-net-coverage-diff} & \UseMacro{apache-commons-net-coverage-exact-same} & \UseMacro{apache-commons-net-coverage-no-stat-sign-diff} \\
\UseMacro{res-apache-commons-pool-name} & \UseMacro{res-apache-commons-pool-bjacoco-min-coverage} & \UseMacro{res-apache-commons-pool-bjacoco-max-coverage} & \UseMacro{res-apache-commons-pool-bjacoco-coverage} & \UseMacro{res-apache-commons-pool-ijacoco-min-coverage} & \UseMacro{res-apache-commons-pool-ijacoco-max-coverage} & \UseMacro{res-apache-commons-pool-ijacoco-coverage} &  \UseMacro{apache-commons-pool-coverage-diff} & \UseMacro{apache-commons-pool-coverage-exact-same} & \UseMacro{apache-commons-pool-coverage-no-stat-sign-diff} \\
\UseMacro{res-alibaba-fastjson-name} & \UseMacro{res-alibaba-fastjson-bjacoco-min-coverage} & \UseMacro{res-alibaba-fastjson-bjacoco-max-coverage} & \UseMacro{res-alibaba-fastjson-bjacoco-coverage} & \UseMacro{res-alibaba-fastjson-ijacoco-min-coverage} & \UseMacro{res-alibaba-fastjson-ijacoco-max-coverage} & \UseMacro{res-alibaba-fastjson-ijacoco-coverage} &  \UseMacro{alibaba-fastjson-coverage-diff} & \UseMacro{alibaba-fastjson-coverage-exact-same} & \UseMacro{alibaba-fastjson-coverage-no-stat-sign-diff} \\
\UseMacro{res-finmath-finmath-lib-name} & \UseMacro{res-finmath-finmath-lib-bjacoco-min-coverage} & \UseMacro{res-finmath-finmath-lib-bjacoco-max-coverage} & \UseMacro{res-finmath-finmath-lib-bjacoco-coverage} & \UseMacro{res-finmath-finmath-lib-ijacoco-min-coverage} & \UseMacro{res-finmath-finmath-lib-ijacoco-max-coverage} & \UseMacro{res-finmath-finmath-lib-ijacoco-coverage} &  \UseMacro{finmath-finmath-lib-coverage-diff} & \UseMacro{finmath-finmath-lib-coverage-exact-same} & \UseMacro{finmath-finmath-lib-coverage-no-stat-sign-diff} \\
\UseMacro{res-sonyxperiadev-gerrit-events-name} & \UseMacro{res-sonyxperiadev-gerrit-events-bjacoco-min-coverage} & \UseMacro{res-sonyxperiadev-gerrit-events-bjacoco-max-coverage} & \UseMacro{res-sonyxperiadev-gerrit-events-bjacoco-coverage} & \UseMacro{res-sonyxperiadev-gerrit-events-ijacoco-min-coverage} & \UseMacro{res-sonyxperiadev-gerrit-events-ijacoco-max-coverage} & \UseMacro{res-sonyxperiadev-gerrit-events-ijacoco-coverage} &  \UseMacro{sonyxperiadev-gerrit-events-coverage-diff} & \UseMacro{sonyxperiadev-gerrit-events-coverage-exact-same} & \UseMacro{sonyxperiadev-gerrit-events-coverage-no-stat-sign-diff} \\
\UseMacro{res-brettwooldridge-HikariCP-name} & \UseMacro{res-brettwooldridge-HikariCP-bjacoco-min-coverage} & \UseMacro{res-brettwooldridge-HikariCP-bjacoco-max-coverage} & \UseMacro{res-brettwooldridge-HikariCP-bjacoco-coverage} & \UseMacro{res-brettwooldridge-HikariCP-ijacoco-min-coverage} & \UseMacro{res-brettwooldridge-HikariCP-ijacoco-max-coverage} & \UseMacro{res-brettwooldridge-HikariCP-ijacoco-coverage} &  \UseMacro{brettwooldridge-HikariCP-coverage-diff} & \UseMacro{brettwooldridge-HikariCP-coverage-exact-same} & \UseMacro{brettwooldridge-HikariCP-coverage-no-stat-sign-diff} \\
\UseMacro{res-lmdbjava-lmdbjava-name} & \UseMacro{res-lmdbjava-lmdbjava-bjacoco-min-coverage} & \UseMacro{res-lmdbjava-lmdbjava-bjacoco-max-coverage} & \UseMacro{res-lmdbjava-lmdbjava-bjacoco-coverage} & \UseMacro{res-lmdbjava-lmdbjava-ijacoco-min-coverage} & \UseMacro{res-lmdbjava-lmdbjava-ijacoco-max-coverage} & \UseMacro{res-lmdbjava-lmdbjava-ijacoco-coverage} &  \UseMacro{lmdbjava-lmdbjava-coverage-diff} & \UseMacro{lmdbjava-lmdbjava-coverage-exact-same} & \UseMacro{lmdbjava-lmdbjava-coverage-no-stat-sign-diff} \\
\UseMacro{res-logic-ng-LogicNG-name} & \UseMacro{res-logic-ng-LogicNG-bjacoco-min-coverage} & \UseMacro{res-logic-ng-LogicNG-bjacoco-max-coverage} & \UseMacro{res-logic-ng-LogicNG-bjacoco-coverage} & \UseMacro{res-logic-ng-LogicNG-ijacoco-min-coverage} & \UseMacro{res-logic-ng-LogicNG-ijacoco-max-coverage} & \UseMacro{res-logic-ng-LogicNG-ijacoco-coverage} &  \UseMacro{logic-ng-LogicNG-coverage-diff} & \UseMacro{logic-ng-LogicNG-coverage-exact-same} & \UseMacro{logic-ng-LogicNG-coverage-no-stat-sign-diff} \\
\UseMacro{res-davidmoten-rxjava-extras-name} & \UseMacro{res-davidmoten-rxjava-extras-bjacoco-min-coverage} & \UseMacro{res-davidmoten-rxjava-extras-bjacoco-max-coverage} & \UseMacro{res-davidmoten-rxjava-extras-bjacoco-coverage} & \UseMacro{res-davidmoten-rxjava-extras-ijacoco-min-coverage} & \UseMacro{res-davidmoten-rxjava-extras-ijacoco-max-coverage} & \UseMacro{res-davidmoten-rxjava-extras-ijacoco-coverage} &  \UseMacro{davidmoten-rxjava-extras-coverage-diff} & \UseMacro{davidmoten-rxjava-extras-coverage-exact-same} & \UseMacro{davidmoten-rxjava-extras-coverage-no-stat-sign-diff} \\
\UseMacro{res-bullhorn-sdk-rest-name} & \UseMacro{res-bullhorn-sdk-rest-bjacoco-min-coverage} & \UseMacro{res-bullhorn-sdk-rest-bjacoco-max-coverage} & \UseMacro{res-bullhorn-sdk-rest-bjacoco-coverage} & \UseMacro{res-bullhorn-sdk-rest-ijacoco-min-coverage} & \UseMacro{res-bullhorn-sdk-rest-ijacoco-max-coverage} & \UseMacro{res-bullhorn-sdk-rest-ijacoco-coverage} &  \UseMacro{bullhorn-sdk-rest-coverage-diff} & \UseMacro{bullhorn-sdk-rest-coverage-exact-same} & \UseMacro{bullhorn-sdk-rest-coverage-no-stat-sign-diff} \\
\UseMacro{res-tabulapdf-tabula-java-name} & \UseMacro{res-tabulapdf-tabula-java-bjacoco-min-coverage} & \UseMacro{res-tabulapdf-tabula-java-bjacoco-max-coverage} & \UseMacro{res-tabulapdf-tabula-java-bjacoco-coverage} & \UseMacro{res-tabulapdf-tabula-java-ijacoco-min-coverage} & \UseMacro{res-tabulapdf-tabula-java-ijacoco-max-coverage} & \UseMacro{res-tabulapdf-tabula-java-ijacoco-coverage} &  \UseMacro{tabulapdf-tabula-java-coverage-diff} & \UseMacro{tabulapdf-tabula-java-coverage-exact-same} & \UseMacro{tabulapdf-tabula-java-coverage-no-stat-sign-diff} \\
\bottomrule \end{tabular}

==> tables/table-results-performance.tex <==
%% Automatically generated by: results.py table_results_performance

\begin{tabular}{l| r|r| r|r| r|r| r|r| r}
\toprule
\multicolumn{1}{c|}{\multirow{3}{*}{\textbf{\UseMacro{TH-project}}}} & \multicolumn{8}{c|}{\textbf{\UseMacro{TH-test-time}}} & \multicolumn{1}{c}{\textbf{\UseMacro{TH-speedup}}} \\
& \multicolumn{2}{c|}{\retestall} & \multicolumn{2}{c|}{\ekstazi} & \multicolumn{2}{c|}{\bjacoco} & \multicolumn{2}{c|}{\ijacocoTool} & \ijacocoTool \\
& \multicolumn{1}{c|}{\UseMacro{TH-avg}} & \multicolumn{1}{c|}{\UseMacro{TH-sum}} & \multicolumn{1}{c|}{\UseMacro{TH-avg}} & \multicolumn{1}{c|}{\UseMacro{TH-sum}} & \multicolumn{1}{c|}{\UseMacro{TH-avg}} & \multicolumn{1}{c|}{\UseMacro{TH-sum}} & \multicolumn{1}{c|}{\UseMacro{TH-avg}} & \multicolumn{1}{c|}{\UseMacro{TH-sum}} & \multicolumn{1}{c}{\UseMacro{TH-avg}}\\
\midrule
\UseMacro{res-asterisk-java-asterisk-java-name} & \UseMacro{res-asterisk-java-asterisk-java-retestall-time} & \UseMacro{res-asterisk-java-asterisk-java-retestall-total-time} & \UseMacro{res-asterisk-java-asterisk-java-ekstazi-time} & \UseMacro{res-asterisk-java-asterisk-java-ekstazi-total-time} & \UseMacro{res-asterisk-java-asterisk-java-bjacoco-time} & \UseMacro{res-asterisk-java-asterisk-java-total-bjacoco-time}  & \UseMacro{res-asterisk-java-asterisk-java-ijacoco-time} & \UseMacro{res-asterisk-java-asterisk-java-total-ijacoco-time} & \UseMacro{res-asterisk-java-asterisk-java-ibjacoco-speedup-time} \\
\UseMacro{res-apache-commons-beanutils-name} & \UseMacro{res-apache-commons-beanutils-retestall-time} & \UseMacro{res-apache-commons-beanutils-retestall-total-time} & \UseMacro{res-apache-commons-beanutils-ekstazi-time} & \UseMacro{res-apache-commons-beanutils-ekstazi-total-time} & \UseMacro{res-apache-commons-beanutils-bjacoco-time} & \UseMacro{res-apache-commons-beanutils-total-bjacoco-time}  & \UseMacro{res-apache-commons-beanutils-ijacoco-time} & \UseMacro{res-apache-commons-beanutils-total-ijacoco-time} & \UseMacro{res-apache-commons-beanutils-ibjacoco-speedup-time} \\
\UseMacro{res-apache-commons-codec-name} & \UseMacro{res-apache-commons-codec-retestall-time} & \UseMacro{res-apache-commons-codec-retestall-total-time} & \UseMacro{res-apache-commons-codec-ekstazi-time} & \UseMacro{res-apache-commons-codec-ekstazi-total-time} & \UseMacro{res-apache-commons-codec-bjacoco-time} & \UseMacro{res-apache-commons-codec-total-bjacoco-time}  & \UseMacro{res-apache-commons-codec-ijacoco-time} & \UseMacro{res-apache-commons-codec-total-ijacoco-time} & \UseMacro{res-apache-commons-codec-ibjacoco-speedup-time} \\
\UseMacro{res-apache-commons-collections-name} & \UseMacro{res-apache-commons-collections-retestall-time} & \UseMacro{res-apache-commons-collections-retestall-total-time} & \UseMacro{res-apache-commons-collections-ekstazi-time} & \UseMacro{res-apache-commons-collections-ekstazi-total-time} & \UseMacro{res-apache-commons-collections-bjacoco-time} & \UseMacro{res-apache-commons-collections-total-bjacoco-time}  & \UseMacro{res-apache-commons-collections-ijacoco-time} & \UseMacro{res-apache-commons-collections-total-ijacoco-time} & \UseMacro{res-apache-commons-collections-ibjacoco-speedup-time} \\
\UseMacro{res-apache-commons-compress-name} & \UseMacro{res-apache-commons-compress-retestall-time} & \UseMacro{res-apache-commons-compress-retestall-total-time} & \UseMacro{res-apache-commons-compress-ekstazi-time} & \UseMacro{res-apache-commons-compress-ekstazi-total-time} & \UseMacro{res-apache-commons-compress-bjacoco-time} & \UseMacro{res-apache-commons-compress-total-bjacoco-time}  & \UseMacro{res-apache-commons-compress-ijacoco-time} & \UseMacro{res-apache-commons-compress-total-ijacoco-time} & \UseMacro{res-apache-commons-compress-ibjacoco-speedup-time} \\
\UseMacro{res-apache-commons-configuration-name} & \UseMacro{res-apache-commons-configuration-retestall-time} & \UseMacro{res-apache-commons-configuration-retestall-total-time} & \UseMacro{res-apache-commons-configuration-ekstazi-time} & \UseMacro{res-apache-commons-configuration-ekstazi-total-time} & \UseMacro{res-apache-commons-configuration-bjacoco-time} & \UseMacro{res-apache-commons-configuration-total-bjacoco-time}  & \UseMacro{res-apache-commons-configuration-ijacoco-time} & \UseMacro{res-apache-commons-configuration-total-ijacoco-time} & \UseMacro{res-apache-commons-configuration-ibjacoco-speedup-time} \\
\UseMacro{res-apache-commons-dbcp-name} & \UseMacro{res-apache-commons-dbcp-retestall-time} & \UseMacro{res-apache-commons-dbcp-retestall-total-time} & \UseMacro{res-apache-commons-dbcp-ekstazi-time} & \UseMacro{res-apache-commons-dbcp-ekstazi-total-time} & \UseMacro{res-apache-commons-dbcp-bjacoco-time} & \UseMacro{res-apache-commons-dbcp-total-bjacoco-time}  & \UseMacro{res-apache-commons-dbcp-ijacoco-time} & \UseMacro{res-apache-commons-dbcp-total-ijacoco-time} & \UseMacro{res-apache-commons-dbcp-ibjacoco-speedup-time} \\
\UseMacro{res-apache-commons-imaging-name} & \UseMacro{res-apache-commons-imaging-retestall-time} & \UseMacro{res-apache-commons-imaging-retestall-total-time} & \UseMacro{res-apache-commons-imaging-ekstazi-time} & \UseMacro{res-apache-commons-imaging-ekstazi-total-time} & \UseMacro{res-apache-commons-imaging-bjacoco-time} & \UseMacro{res-apache-commons-imaging-total-bjacoco-time}  & \UseMacro{res-apache-commons-imaging-ijacoco-time} & \UseMacro{res-apache-commons-imaging-total-ijacoco-time} & \UseMacro{res-apache-commons-imaging-ibjacoco-speedup-time} \\
\UseMacro{res-apache-commons-io-name} & \UseMacro{res-apache-commons-io-retestall-time} & \UseMacro{res-apache-commons-io-retestall-total-time} & \UseMacro{res-apache-commons-io-ekstazi-time} & \UseMacro{res-apache-commons-io-ekstazi-total-time} & \UseMacro{res-apache-commons-io-bjacoco-time} & \UseMacro{res-apache-commons-io-total-bjacoco-time}  & \UseMacro{res-apache-commons-io-ijacoco-time} & \UseMacro{res-apache-commons-io-total-ijacoco-time} & \UseMacro{res-apache-commons-io-ibjacoco-speedup-time} \\
\UseMacro{res-apache-commons-lang-name} & \UseMacro{res-apache-commons-lang-retestall-time} & \UseMacro{res-apache-commons-lang-retestall-total-time} & \UseMacro{res-apache-commons-lang-ekstazi-time} & \UseMacro{res-apache-commons-lang-ekstazi-total-time} & \UseMacro{res-apache-commons-lang-bjacoco-time} & \UseMacro{res-apache-commons-lang-total-bjacoco-time}  & \UseMacro{res-apache-commons-lang-ijacoco-time} & \UseMacro{res-apache-commons-lang-total-ijacoco-time} & \UseMacro{res-apache-commons-lang-ibjacoco-speedup-time} \\
\UseMacro{res-apache-commons-math-name} & \UseMacro{res-apache-commons-math-retestall-time} & \UseMacro{res-apache-commons-math-retestall-total-time} & \UseMacro{res-apache-commons-math-ekstazi-time} & \UseMacro{res-apache-commons-math-ekstazi-total-time} & \UseMacro{res-apache-commons-math-bjacoco-time} & \UseMacro{res-apache-commons-math-total-bjacoco-time}  & \UseMacro{res-apache-commons-math-ijacoco-time} & \UseMacro{res-apache-commons-math-total-ijacoco-time} & \UseMacro{res-apache-commons-math-ibjacoco-speedup-time} \\
\UseMacro{res-apache-commons-net-name} & \UseMacro{res-apache-commons-net-retestall-time} & \UseMacro{res-apache-commons-net-retestall-total-time} & \UseMacro{res-apache-commons-net-ekstazi-time} & \UseMacro{res-apache-commons-net-ekstazi-total-time} & \UseMacro{res-apache-commons-net-bjacoco-time} & \UseMacro{res-apache-commons-net-total-bjacoco-time}  & \UseMacro{res-apache-commons-net-ijacoco-time} & \UseMacro{res-apache-commons-net-total-ijacoco-time} & \UseMacro{res-apache-commons-net-ibjacoco-speedup-time} \\
\UseMacro{res-apache-commons-pool-name} & \UseMacro{res-apache-commons-pool-retestall-time} & \UseMacro{res-apache-commons-pool-retestall-total-time} & \UseMacro{res-apache-commons-pool-ekstazi-time} & \UseMacro{res-apache-commons-pool-ekstazi-total-time} & \UseMacro{res-apache-commons-pool-bjacoco-time} & \UseMacro{res-apache-commons-pool-total-bjacoco-time}  & \UseMacro{res-apache-commons-pool-ijacoco-time} & \UseMacro{res-apache-commons-pool-total-ijacoco-time} & \UseMacro{res-apache-commons-pool-ibjacoco-speedup-time} \\
\UseMacro{res-alibaba-fastjson-name} & \UseMacro{res-alibaba-fastjson-retestall-time} & \UseMacro{res-alibaba-fastjson-retestall-total-time} & \UseMacro{res-alibaba-fastjson-ekstazi-time} & \UseMacro{res-alibaba-fastjson-ekstazi-total-time} & \UseMacro{res-alibaba-fastjson-bjacoco-time} & \UseMacro{res-alibaba-fastjson-total-bjacoco-time}  & \UseMacro{res-alibaba-fastjson-ijacoco-time} & \UseMacro{res-alibaba-fastjson-total-ijacoco-time} & \UseMacro{res-alibaba-fastjson-ibjacoco-speedup-time} \\
\UseMacro{res-finmath-finmath-lib-name} & \UseMacro{res-finmath-finmath-lib-retestall-time} & \UseMacro{res-finmath-finmath-lib-retestall-total-time} & \UseMacro{res-finmath-finmath-lib-ekstazi-time} & \UseMacro{res-finmath-finmath-lib-ekstazi-total-time} & \UseMacro{res-finmath-finmath-lib-bjacoco-time} & \UseMacro{res-finmath-finmath-lib-total-bjacoco-time}  & \UseMacro{res-finmath-finmath-lib-ijacoco-time} & \UseMacro{res-finmath-finmath-lib-total-ijacoco-time} & \UseMacro{res-finmath-finmath-lib-ibjacoco-speedup-time} \\
\UseMacro{res-sonyxperiadev-gerrit-events-name} & \UseMacro{res-sonyxperiadev-gerrit-events-retestall-time} & \UseMacro{res-sonyxperiadev-gerrit-events-retestall-total-time} & \UseMacro{res-sonyxperiadev-gerrit-events-ekstazi-time} & \UseMacro{res-sonyxperiadev-gerrit-events-ekstazi-total-time} & \UseMacro{res-sonyxperiadev-gerrit-events-bjacoco-time} & \UseMacro{res-sonyxperiadev-gerrit-events-total-bjacoco-time}  & \UseMacro{res-sonyxperiadev-gerrit-events-ijacoco-time} & \UseMacro{res-sonyxperiadev-gerrit-events-total-ijacoco-time} & \UseMacro{res-sonyxperiadev-gerrit-events-ibjacoco-speedup-time} \\
\UseMacro{res-brettwooldridge-HikariCP-name} & \UseMacro{res-brettwooldridge-HikariCP-retestall-time} & \UseMacro{res-brettwooldridge-HikariCP-retestall-total-time} & \UseMacro{res-brettwooldridge-HikariCP-ekstazi-time} & \UseMacro{res-brettwooldridge-HikariCP-ekstazi-total-time} & \UseMacro{res-brettwooldridge-HikariCP-bjacoco-time} & \UseMacro{res-brettwooldridge-HikariCP-total-bjacoco-time}  & \UseMacro{res-brettwooldridge-HikariCP-ijacoco-time} & \UseMacro{res-brettwooldridge-HikariCP-total-ijacoco-time} & \UseMacro{res-brettwooldridge-HikariCP-ibjacoco-speedup-time} \\
\UseMacro{res-lmdbjava-lmdbjava-name} & \UseMacro{res-lmdbjava-lmdbjava-retestall-time} & \UseMacro{res-lmdbjava-lmdbjava-retestall-total-time} & \UseMacro{res-lmdbjava-lmdbjava-ekstazi-time} & \UseMacro{res-lmdbjava-lmdbjava-ekstazi-total-time} & \UseMacro{res-lmdbjava-lmdbjava-bjacoco-time} & \UseMacro{res-lmdbjava-lmdbjava-total-bjacoco-time}  & \UseMacro{res-lmdbjava-lmdbjava-ijacoco-time} & \UseMacro{res-lmdbjava-lmdbjava-total-ijacoco-time} & \UseMacro{res-lmdbjava-lmdbjava-ibjacoco-speedup-time} \\
\UseMacro{res-logic-ng-LogicNG-name} & \UseMacro{res-logic-ng-LogicNG-retestall-time} & \UseMacro{res-logic-ng-LogicNG-retestall-total-time} & \UseMacro{res-logic-ng-LogicNG-ekstazi-time} & \UseMacro{res-logic-ng-LogicNG-ekstazi-total-time} & \UseMacro{res-logic-ng-LogicNG-bjacoco-time} & \UseMacro{res-logic-ng-LogicNG-total-bjacoco-time}  & \UseMacro{res-logic-ng-LogicNG-ijacoco-time} & \UseMacro{res-logic-ng-LogicNG-total-ijacoco-time} & \UseMacro{res-logic-ng-LogicNG-ibjacoco-speedup-time} \\
\UseMacro{res-davidmoten-rxjava-extras-name} & \UseMacro{res-davidmoten-rxjava-extras-retestall-time} & \UseMacro{res-davidmoten-rxjava-extras-retestall-total-time} & \UseMacro{res-davidmoten-rxjava-extras-ekstazi-time} & \UseMacro{res-davidmoten-rxjava-extras-ekstazi-total-time} & \UseMacro{res-davidmoten-rxjava-extras-bjacoco-time} & \UseMacro{res-davidmoten-rxjava-extras-total-bjacoco-time}  & \UseMacro{res-davidmoten-rxjava-extras-ijacoco-time} & \UseMacro{res-davidmoten-rxjava-extras-total-ijacoco-time} & \UseMacro{res-davidmoten-rxjava-extras-ibjacoco-speedup-time} \\
\UseMacro{res-bullhorn-sdk-rest-name} & \UseMacro{res-bullhorn-sdk-rest-retestall-time} & \UseMacro{res-bullhorn-sdk-rest-retestall-total-time} & \UseMacro{res-bullhorn-sdk-rest-ekstazi-time} & \UseMacro{res-bullhorn-sdk-rest-ekstazi-total-time} & \UseMacro{res-bullhorn-sdk-rest-bjacoco-time} & \UseMacro{res-bullhorn-sdk-rest-total-bjacoco-time}  & \UseMacro{res-bullhorn-sdk-rest-ijacoco-time} & \UseMacro{res-bullhorn-sdk-rest-total-ijacoco-time} & \UseMacro{res-bullhorn-sdk-rest-ibjacoco-speedup-time} \\
\UseMacro{res-tabulapdf-tabula-java-name} & \UseMacro{res-tabulapdf-tabula-java-retestall-time} & \UseMacro{res-tabulapdf-tabula-java-retestall-total-time} & \UseMacro{res-tabulapdf-tabula-java-ekstazi-time} & \UseMacro{res-tabulapdf-tabula-java-ekstazi-total-time} & \UseMacro{res-tabulapdf-tabula-java-bjacoco-time} & \UseMacro{res-tabulapdf-tabula-java-total-bjacoco-time}  & \UseMacro{res-tabulapdf-tabula-java-ijacoco-time} & \UseMacro{res-tabulapdf-tabula-java-total-ijacoco-time} & \UseMacro{res-tabulapdf-tabula-java-ibjacoco-speedup-time} \\
\midrule
\multicolumn{1}{c|}{\textbf{\UseMacro{TH-avg}}} &  \UseMacro{retestall-avg-time} & \UseMacro{retestall-avg-total-time} & \UseMacro{ekstazi-avg-time} & \UseMacro{ekstazi-avg-total-time} & \UseMacro{bjacoco-avg-time} & \UseMacro{bjacoco-avg-total-time}  & \UseMacro{ijacoco-avg-time} & \UseMacro{ijacoco-avg-total-time} & \UseMacro{ijacoco-avg-speedup} \\ 
\bottomrule \end{tabular}

==> tables/table-results-phase-time.tex <==
%% Automatically generated by: results.py table_results_phase_time

\begin{tabular}{l|r|r|r|r}
\toprule
\multicolumn{1}{c|}{\multirow{3}{*}{\textbf{\UseMacro{TH-project}}}} & \multicolumn{4}{c}{\textbf{\UseMacro{TH-phase-time}}} \\
 & \UseMacro{TH-compile-time} & \UseMacro{TH-analysis-time} & \UseMacro{TH-execution-collection-time} & \UseMacro{TH-report-time}\\ 
\midrule
\UseMacro{res-asterisk-java-asterisk-java-name} & \UseMacro{res-asterisk-java-asterisk-java-phase-compile} (\UseMacro{res-asterisk-java-asterisk-java-phase-compile-percent}\%) & \UseMacro{res-asterisk-java-asterisk-java-phase-analysis} (\UseMacro{res-asterisk-java-asterisk-java-phase-analysis-percent}\%) & \UseMacro{res-asterisk-java-asterisk-java-phase-execution-collection} (\UseMacro{res-asterisk-java-asterisk-java-phase-execution-collection-percent}\%) & \UseMacro{res-asterisk-java-asterisk-java-phase-report} (\UseMacro{res-asterisk-java-asterisk-java-phase-report-percent}\%)\\
\UseMacro{res-apache-commons-beanutils-name} & \UseMacro{res-apache-commons-beanutils-phase-compile} (\UseMacro{res-apache-commons-beanutils-phase-compile-percent}\%) & \UseMacro{res-apache-commons-beanutils-phase-analysis} (\UseMacro{res-apache-commons-beanutils-phase-analysis-percent}\%) & \UseMacro{res-apache-commons-beanutils-phase-execution-collection} (\UseMacro{res-apache-commons-beanutils-phase-execution-collection-percent}\%) & \UseMacro{res-apache-commons-beanutils-phase-report} (\UseMacro{res-apache-commons-beanutils-phase-report-percent}\%)\\
\UseMacro{res-apache-commons-codec-name} & \UseMacro{res-apache-commons-codec-phase-compile} (\UseMacro{res-apache-commons-codec-phase-compile-percent}\%) & \UseMacro{res-apache-commons-codec-phase-analysis} (\UseMacro{res-apache-commons-codec-phase-analysis-percent}\%) & \UseMacro{res-apache-commons-codec-phase-execution-collection} (\UseMacro{res-apache-commons-codec-phase-execution-collection-percent}\%) & \UseMacro{res-apache-commons-codec-phase-report} (\UseMacro{res-apache-commons-codec-phase-report-percent}\%)\\
\UseMacro{res-apache-commons-collections-name} & \UseMacro{res-apache-commons-collections-phase-compile} (\UseMacro{res-apache-commons-collections-phase-compile-percent}\%) & \UseMacro{res-apache-commons-collections-phase-analysis} (\UseMacro{res-apache-commons-collections-phase-analysis-percent}\%) & \UseMacro{res-apache-commons-collections-phase-execution-collection} (\UseMacro{res-apache-commons-collections-phase-execution-collection-percent}\%) & \UseMacro{res-apache-commons-collections-phase-report} (\UseMacro{res-apache-commons-collections-phase-report-percent}\%)\\
\UseMacro{res-apache-commons-compress-name} & \UseMacro{res-apache-commons-compress-phase-compile} (\UseMacro{res-apache-commons-compress-phase-compile-percent}\%) & \UseMacro{res-apache-commons-compress-phase-analysis} (\UseMacro{res-apache-commons-compress-phase-analysis-percent}\%) & \UseMacro{res-apache-commons-compress-phase-execution-collection} (\UseMacro{res-apache-commons-compress-phase-execution-collection-percent}\%) & \UseMacro{res-apache-commons-compress-phase-report} (\UseMacro{res-apache-commons-compress-phase-report-percent}\%)\\
\UseMacro{res-apache-commons-configuration-name} & \UseMacro{res-apache-commons-configuration-phase-compile} (\UseMacro{res-apache-commons-configuration-phase-compile-percent}\%) & \UseMacro{res-apache-commons-configuration-phase-analysis} (\UseMacro{res-apache-commons-configuration-phase-analysis-percent}\%) & \UseMacro{res-apache-commons-configuration-phase-execution-collection} (\UseMacro{res-apache-commons-configuration-phase-execution-collection-percent}\%) & \UseMacro{res-apache-commons-configuration-phase-report} (\UseMacro{res-apache-commons-configuration-phase-report-percent}\%)\\
\UseMacro{res-apache-commons-dbcp-name} & \UseMacro{res-apache-commons-dbcp-phase-compile} (\UseMacro{res-apache-commons-dbcp-phase-compile-percent}\%) & \UseMacro{res-apache-commons-dbcp-phase-analysis} (\UseMacro{res-apache-commons-dbcp-phase-analysis-percent}\%) & \UseMacro{res-apache-commons-dbcp-phase-execution-collection} (\UseMacro{res-apache-commons-dbcp-phase-execution-collection-percent}\%) & \UseMacro{res-apache-commons-dbcp-phase-report} (\UseMacro{res-apache-commons-dbcp-phase-report-percent}\%)\\
\UseMacro{res-apache-commons-imaging-name} & \UseMacro{res-apache-commons-imaging-phase-compile} (\UseMacro{res-apache-commons-imaging-phase-compile-percent}\%) & \UseMacro{res-apache-commons-imaging-phase-analysis} (\UseMacro{res-apache-commons-imaging-phase-analysis-percent}\%) & \UseMacro{res-apache-commons-imaging-phase-execution-collection} (\UseMacro{res-apache-commons-imaging-phase-execution-collection-percent}\%) & \UseMacro{res-apache-commons-imaging-phase-report} (\UseMacro{res-apache-commons-imaging-phase-report-percent}\%)\\
\UseMacro{res-apache-commons-io-name} & \UseMacro{res-apache-commons-io-phase-compile} (\UseMacro{res-apache-commons-io-phase-compile-percent}\%) & \UseMacro{res-apache-commons-io-phase-analysis} (\UseMacro{res-apache-commons-io-phase-analysis-percent}\%) & \UseMacro{res-apache-commons-io-phase-execution-collection} (\UseMacro{res-apache-commons-io-phase-execution-collection-percent}\%) & \UseMacro{res-apache-commons-io-phase-report} (\UseMacro{res-apache-commons-io-phase-report-percent}\%)\\
\UseMacro{res-apache-commons-lang-name} & \UseMacro{res-apache-commons-lang-phase-compile} (\UseMacro{res-apache-commons-lang-phase-compile-percent}\%) & \UseMacro{res-apache-commons-lang-phase-analysis} (\UseMacro{res-apache-commons-lang-phase-analysis-percent}\%) & \UseMacro{res-apache-commons-lang-phase-execution-collection} (\UseMacro{res-apache-commons-lang-phase-execution-collection-percent}\%) & \UseMacro{res-apache-commons-lang-phase-report} (\UseMacro{res-apache-commons-lang-phase-report-percent}\%)\\
\UseMacro{res-apache-commons-math-name} & \UseMacro{res-apache-commons-math-phase-compile} (\UseMacro{res-apache-commons-math-phase-compile-percent}\%) & \UseMacro{res-apache-commons-math-phase-analysis} (\UseMacro{res-apache-commons-math-phase-analysis-percent}\%) & \UseMacro{res-apache-commons-math-phase-execution-collection} (\UseMacro{res-apache-commons-math-phase-execution-collection-percent}\%) & \UseMacro{res-apache-commons-math-phase-report} (\UseMacro{res-apache-commons-math-phase-report-percent}\%)\\
\UseMacro{res-apache-commons-net-name} & \UseMacro{res-apache-commons-net-phase-compile} (\UseMacro{res-apache-commons-net-phase-compile-percent}\%) & \UseMacro{res-apache-commons-net-phase-analysis} (\UseMacro{res-apache-commons-net-phase-analysis-percent}\%) & \UseMacro{res-apache-commons-net-phase-execution-collection} (\UseMacro{res-apache-commons-net-phase-execution-collection-percent}\%) & \UseMacro{res-apache-commons-net-phase-report} (\UseMacro{res-apache-commons-net-phase-report-percent}\%)\\
\UseMacro{res-apache-commons-pool-name} & \UseMacro{res-apache-commons-pool-phase-compile} (\UseMacro{res-apache-commons-pool-phase-compile-percent}\%) & \UseMacro{res-apache-commons-pool-phase-analysis} (\UseMacro{res-apache-commons-pool-phase-analysis-percent}\%) & \UseMacro{res-apache-commons-pool-phase-execution-collection} (\UseMacro{res-apache-commons-pool-phase-execution-collection-percent}\%) & \UseMacro{res-apache-commons-pool-phase-report} (\UseMacro{res-apache-commons-pool-phase-report-percent}\%)\\
\UseMacro{res-alibaba-fastjson-name} & \UseMacro{res-alibaba-fastjson-phase-compile} (\UseMacro{res-alibaba-fastjson-phase-compile-percent}\%) & \UseMacro{res-alibaba-fastjson-phase-analysis} (\UseMacro{res-alibaba-fastjson-phase-analysis-percent}\%) & \UseMacro{res-alibaba-fastjson-phase-execution-collection} (\UseMacro{res-alibaba-fastjson-phase-execution-collection-percent}\%) & \UseMacro{res-alibaba-fastjson-phase-report} (\UseMacro{res-alibaba-fastjson-phase-report-percent}\%)\\
\UseMacro{res-finmath-finmath-lib-name} & \UseMacro{res-finmath-finmath-lib-phase-compile} (\UseMacro{res-finmath-finmath-lib-phase-compile-percent}\%) & \UseMacro{res-finmath-finmath-lib-phase-analysis} (\UseMacro{res-finmath-finmath-lib-phase-analysis-percent}\%) & \UseMacro{res-finmath-finmath-lib-phase-execution-collection} (\UseMacro{res-finmath-finmath-lib-phase-execution-collection-percent}\%) & \UseMacro{res-finmath-finmath-lib-phase-report} (\UseMacro{res-finmath-finmath-lib-phase-report-percent}\%)\\
\UseMacro{res-sonyxperiadev-gerrit-events-name} & \UseMacro{res-sonyxperiadev-gerrit-events-phase-compile} (\UseMacro{res-sonyxperiadev-gerrit-events-phase-compile-percent}\%) & \UseMacro{res-sonyxperiadev-gerrit-events-phase-analysis} (\UseMacro{res-sonyxperiadev-gerrit-events-phase-analysis-percent}\%) & \UseMacro{res-sonyxperiadev-gerrit-events-phase-execution-collection} (\UseMacro{res-sonyxperiadev-gerrit-events-phase-execution-collection-percent}\%) & \UseMacro{res-sonyxperiadev-gerrit-events-phase-report} (\UseMacro{res-sonyxperiadev-gerrit-events-phase-report-percent}\%)\\
\UseMacro{res-brettwooldridge-HikariCP-name} & \UseMacro{res-brettwooldridge-HikariCP-phase-compile} (\UseMacro{res-brettwooldridge-HikariCP-phase-compile-percent}\%) & \UseMacro{res-brettwooldridge-HikariCP-phase-analysis} (\UseMacro{res-brettwooldridge-HikariCP-phase-analysis-percent}\%) & \UseMacro{res-brettwooldridge-HikariCP-phase-execution-collection} (\UseMacro{res-brettwooldridge-HikariCP-phase-execution-collection-percent}\%) & \UseMacro{res-brettwooldridge-HikariCP-phase-report} (\UseMacro{res-brettwooldridge-HikariCP-phase-report-percent}\%)\\
\UseMacro{res-lmdbjava-lmdbjava-name} & \UseMacro{res-lmdbjava-lmdbjava-phase-compile} (\UseMacro{res-lmdbjava-lmdbjava-phase-compile-percent}\%) & \UseMacro{res-lmdbjava-lmdbjava-phase-analysis} (\UseMacro{res-lmdbjava-lmdbjava-phase-analysis-percent}\%) & \UseMacro{res-lmdbjava-lmdbjava-phase-execution-collection} (\UseMacro{res-lmdbjava-lmdbjava-phase-execution-collection-percent}\%) & \UseMacro{res-lmdbjava-lmdbjava-phase-report} (\UseMacro{res-lmdbjava-lmdbjava-phase-report-percent}\%)\\
\UseMacro{res-logic-ng-LogicNG-name} & \UseMacro{res-logic-ng-LogicNG-phase-compile} (\UseMacro{res-logic-ng-LogicNG-phase-compile-percent}\%) & \UseMacro{res-logic-ng-LogicNG-phase-analysis} (\UseMacro{res-logic-ng-LogicNG-phase-analysis-percent}\%) & \UseMacro{res-logic-ng-LogicNG-phase-execution-collection} (\UseMacro{res-logic-ng-LogicNG-phase-execution-collection-percent}\%) & \UseMacro{res-logic-ng-LogicNG-phase-report} (\UseMacro{res-logic-ng-LogicNG-phase-report-percent}\%)\\
\UseMacro{res-davidmoten-rxjava-extras-name} & \UseMacro{res-davidmoten-rxjava-extras-phase-compile} (\UseMacro{res-davidmoten-rxjava-extras-phase-compile-percent}\%) & \UseMacro{res-davidmoten-rxjava-extras-phase-analysis} (\UseMacro{res-davidmoten-rxjava-extras-phase-analysis-percent}\%) & \UseMacro{res-davidmoten-rxjava-extras-phase-execution-collection} (\UseMacro{res-davidmoten-rxjava-extras-phase-execution-collection-percent}\%) & \UseMacro{res-davidmoten-rxjava-extras-phase-report} (\UseMacro{res-davidmoten-rxjava-extras-phase-report-percent}\%)\\
\UseMacro{res-bullhorn-sdk-rest-name} & \UseMacro{res-bullhorn-sdk-rest-phase-compile} (\UseMacro{res-bullhorn-sdk-rest-phase-compile-percent}\%) & \UseMacro{res-bullhorn-sdk-rest-phase-analysis} (\UseMacro{res-bullhorn-sdk-rest-phase-analysis-percent}\%) & \UseMacro{res-bullhorn-sdk-rest-phase-execution-collection} (\UseMacro{res-bullhorn-sdk-rest-phase-execution-collection-percent}\%) & \UseMacro{res-bullhorn-sdk-rest-phase-report} (\UseMacro{res-bullhorn-sdk-rest-phase-report-percent}\%)\\
\UseMacro{res-tabulapdf-tabula-java-name} & \UseMacro{res-tabulapdf-tabula-java-phase-compile} (\UseMacro{res-tabulapdf-tabula-java-phase-compile-percent}\%) & \UseMacro{res-tabulapdf-tabula-java-phase-analysis} (\UseMacro{res-tabulapdf-tabula-java-phase-analysis-percent}\%) & \UseMacro{res-tabulapdf-tabula-java-phase-execution-collection} (\UseMacro{res-tabulapdf-tabula-java-phase-execution-collection-percent}\%) & \UseMacro{res-tabulapdf-tabula-java-phase-report} (\UseMacro{res-tabulapdf-tabula-java-phase-report-percent}\%)\\
\midrule
\multicolumn{1}{c|}{{\textbf{\UseMacro{TH-avg}}}} & \UseMacro{res-phase-avg-compile} (\UseMacro{res-phase-avg-compile-percent}\%) & \UseMacro{res-phase-avg-analysis} (\UseMacro{res-phase-avg-analysis-percent}\%) & \UseMacro{res-phase-avg-execution-collection} (\UseMacro{res-phase-avg-execution-collection-percent}\%) & \UseMacro{res-phase-avg-report} (\UseMacro{res-phase-avg-report-percent}\%)\\ 
\bottomrule\end{tabular}

==> tables/table-results-selected-test-and-phase-time.tex <==
%% Automatically generated by: results.py table_results_selected_test_and_phase_time

\begin{tabular}{l|r|r|r|r|r|r}
\toprule
\multicolumn{1}{c|}{\multirow{3}{*}{\textbf{\UseMacro{TH-project}}}} & \multicolumn{2}{c|}{\textbf{\UseMacro{TH-selected-test-ratio}}} & \multicolumn{4}{c}{\textbf{\UseMacro{TH-phase-time}}} \\
 & \multicolumn{1}{c|}{\ekstazi} & \multicolumn{1}{c|}{\ijacocoTool} & \multicolumn{1}{c|}{\UseMacro{TH-compile-time}} & \multicolumn{1}{c|}{\UseMacro{TH-analysis-time}} & \multicolumn{1}{c|}{\UseMacro{TH-execution-collection-time}} & \multicolumn{1}{c}{\UseMacro{TH-report-time}} \\ 
\midrule
\UseMacro{res-asterisk-java-asterisk-java-name} & \UseMacro{res-asterisk-java-asterisk-java-ekstazi-selected-rate} & \UseMacro{res-asterisk-java-asterisk-java-ijacoco-selected-rate} & \UseMacro{res-asterisk-java-asterisk-java-phase-compile} (\UseMacro{res-asterisk-java-asterisk-java-phase-compile-percent}\%) & \UseMacro{res-asterisk-java-asterisk-java-phase-analysis} (\UseMacro{res-asterisk-java-asterisk-java-phase-analysis-percent}\%) & \UseMacro{res-asterisk-java-asterisk-java-phase-execution-collection} (\UseMacro{res-asterisk-java-asterisk-java-phase-execution-collection-percent}\%) & \UseMacro{res-asterisk-java-asterisk-java-phase-report} (\UseMacro{res-asterisk-java-asterisk-java-phase-report-percent}\%)\\
\UseMacro{res-apache-commons-beanutils-name} & \UseMacro{res-apache-commons-beanutils-ekstazi-selected-rate} & \UseMacro{res-apache-commons-beanutils-ijacoco-selected-rate} & \UseMacro{res-apache-commons-beanutils-phase-compile} (\UseMacro{res-apache-commons-beanutils-phase-compile-percent}\%) & \UseMacro{res-apache-commons-beanutils-phase-analysis} (\UseMacro{res-apache-commons-beanutils-phase-analysis-percent}\%) & \UseMacro{res-apache-commons-beanutils-phase-execution-collection} (\UseMacro{res-apache-commons-beanutils-phase-execution-collection-percent}\%) & \UseMacro{res-apache-commons-beanutils-phase-report} (\UseMacro{res-apache-commons-beanutils-phase-report-percent}\%)\\
\UseMacro{res-apache-commons-codec-name} & \UseMacro{res-apache-commons-codec-ekstazi-selected-rate} & \UseMacro{res-apache-commons-codec-ijacoco-selected-rate} & \UseMacro{res-apache-commons-codec-phase-compile} (\UseMacro{res-apache-commons-codec-phase-compile-percent}\%) & \UseMacro{res-apache-commons-codec-phase-analysis} (\UseMacro{res-apache-commons-codec-phase-analysis-percent}\%) & \UseMacro{res-apache-commons-codec-phase-execution-collection} (\UseMacro{res-apache-commons-codec-phase-execution-collection-percent}\%) & \UseMacro{res-apache-commons-codec-phase-report} (\UseMacro{res-apache-commons-codec-phase-report-percent}\%)\\
\UseMacro{res-apache-commons-collections-name} & \UseMacro{res-apache-commons-collections-ekstazi-selected-rate} & \UseMacro{res-apache-commons-collections-ijacoco-selected-rate} & \UseMacro{res-apache-commons-collections-phase-compile} (\UseMacro{res-apache-commons-collections-phase-compile-percent}\%) & \UseMacro{res-apache-commons-collections-phase-analysis} (\UseMacro{res-apache-commons-collections-phase-analysis-percent}\%) & \UseMacro{res-apache-commons-collections-phase-execution-collection} (\UseMacro{res-apache-commons-collections-phase-execution-collection-percent}\%) & \UseMacro{res-apache-commons-collections-phase-report} (\UseMacro{res-apache-commons-collections-phase-report-percent}\%)\\
\UseMacro{res-apache-commons-compress-name} & \UseMacro{res-apache-commons-compress-ekstazi-selected-rate} & \UseMacro{res-apache-commons-compress-ijacoco-selected-rate} & \UseMacro{res-apache-commons-compress-phase-compile} (\UseMacro{res-apache-commons-compress-phase-compile-percent}\%) & \UseMacro{res-apache-commons-compress-phase-analysis} (\UseMacro{res-apache-commons-compress-phase-analysis-percent}\%) & \UseMacro{res-apache-commons-compress-phase-execution-collection} (\UseMacro{res-apache-commons-compress-phase-execution-collection-percent}\%) & \UseMacro{res-apache-commons-compress-phase-report} (\UseMacro{res-apache-commons-compress-phase-report-percent}\%)\\
\UseMacro{res-apache-commons-configuration-name} & \UseMacro{res-apache-commons-configuration-ekstazi-selected-rate} & \UseMacro{res-apache-commons-configuration-ijacoco-selected-rate} & \UseMacro{res-apache-commons-configuration-phase-compile} (\UseMacro{res-apache-commons-configuration-phase-compile-percent}\%) & \UseMacro{res-apache-commons-configuration-phase-analysis} (\UseMacro{res-apache-commons-configuration-phase-analysis-percent}\%) & \UseMacro{res-apache-commons-configuration-phase-execution-collection} (\UseMacro{res-apache-commons-configuration-phase-execution-collection-percent}\%) & \UseMacro{res-apache-commons-configuration-phase-report} (\UseMacro{res-apache-commons-configuration-phase-report-percent}\%)\\
\UseMacro{res-apache-commons-dbcp-name} & \UseMacro{res-apache-commons-dbcp-ekstazi-selected-rate} & \UseMacro{res-apache-commons-dbcp-ijacoco-selected-rate} & \UseMacro{res-apache-commons-dbcp-phase-compile} (\UseMacro{res-apache-commons-dbcp-phase-compile-percent}\%) & \UseMacro{res-apache-commons-dbcp-phase-analysis} (\UseMacro{res-apache-commons-dbcp-phase-analysis-percent}\%) & \UseMacro{res-apache-commons-dbcp-phase-execution-collection} (\UseMacro{res-apache-commons-dbcp-phase-execution-collection-percent}\%) & \UseMacro{res-apache-commons-dbcp-phase-report} (\UseMacro{res-apache-commons-dbcp-phase-report-percent}\%)\\
\UseMacro{res-apache-commons-imaging-name} & \UseMacro{res-apache-commons-imaging-ekstazi-selected-rate} & \UseMacro{res-apache-commons-imaging-ijacoco-selected-rate} & \UseMacro{res-apache-commons-imaging-phase-compile} (\UseMacro{res-apache-commons-imaging-phase-compile-percent}\%) & \UseMacro{res-apache-commons-imaging-phase-analysis} (\UseMacro{res-apache-commons-imaging-phase-analysis-percent}\%) & \UseMacro{res-apache-commons-imaging-phase-execution-collection} (\UseMacro{res-apache-commons-imaging-phase-execution-collection-percent}\%) & \UseMacro{res-apache-commons-imaging-phase-report} (\UseMacro{res-apache-commons-imaging-phase-report-percent}\%)\\
\UseMacro{res-apache-commons-io-name} & \UseMacro{res-apache-commons-io-ekstazi-selected-rate} & \UseMacro{res-apache-commons-io-ijacoco-selected-rate} & \UseMacro{res-apache-commons-io-phase-compile} (\UseMacro{res-apache-commons-io-phase-compile-percent}\%) & \UseMacro{res-apache-commons-io-phase-analysis} (\UseMacro{res-apache-commons-io-phase-analysis-percent}\%) & \UseMacro{res-apache-commons-io-phase-execution-collection} (\UseMacro{res-apache-commons-io-phase-execution-collection-percent}\%) & \UseMacro{res-apache-commons-io-phase-report} (\UseMacro{res-apache-commons-io-phase-report-percent}\%)\\
\UseMacro{res-apache-commons-lang-name} & \UseMacro{res-apache-commons-lang-ekstazi-selected-rate} & \UseMacro{res-apache-commons-lang-ijacoco-selected-rate} & \UseMacro{res-apache-commons-lang-phase-compile} (\UseMacro{res-apache-commons-lang-phase-compile-percent}\%) & \UseMacro{res-apache-commons-lang-phase-analysis} (\UseMacro{res-apache-commons-lang-phase-analysis-percent}\%) & \UseMacro{res-apache-commons-lang-phase-execution-collection} (\UseMacro{res-apache-commons-lang-phase-execution-collection-percent}\%) & \UseMacro{res-apache-commons-lang-phase-report} (\UseMacro{res-apache-commons-lang-phase-report-percent}\%)\\
\UseMacro{res-apache-commons-math-name} & \UseMacro{res-apache-commons-math-ekstazi-selected-rate} & \UseMacro{res-apache-commons-math-ijacoco-selected-rate} & \UseMacro{res-apache-commons-math-phase-compile} (\UseMacro{res-apache-commons-math-phase-compile-percent}\%) & \UseMacro{res-apache-commons-math-phase-analysis} (\UseMacro{res-apache-commons-math-phase-analysis-percent}\%) & \UseMacro{res-apache-commons-math-phase-execution-collection} (\UseMacro{res-apache-commons-math-phase-execution-collection-percent}\%) & \UseMacro{res-apache-commons-math-phase-report} (\UseMacro{res-apache-commons-math-phase-report-percent}\%)\\
\UseMacro{res-apache-commons-net-name} & \UseMacro{res-apache-commons-net-ekstazi-selected-rate} & \UseMacro{res-apache-commons-net-ijacoco-selected-rate} & \UseMacro{res-apache-commons-net-phase-compile} (\UseMacro{res-apache-commons-net-phase-compile-percent}\%) & \UseMacro{res-apache-commons-net-phase-analysis} (\UseMacro{res-apache-commons-net-phase-analysis-percent}\%) & \UseMacro{res-apache-commons-net-phase-execution-collection} (\UseMacro{res-apache-commons-net-phase-execution-collection-percent}\%) & \UseMacro{res-apache-commons-net-phase-report} (\UseMacro{res-apache-commons-net-phase-report-percent}\%)\\
\UseMacro{res-apache-commons-pool-name} & \UseMacro{res-apache-commons-pool-ekstazi-selected-rate} & \UseMacro{res-apache-commons-pool-ijacoco-selected-rate} & \UseMacro{res-apache-commons-pool-phase-compile} (\UseMacro{res-apache-commons-pool-phase-compile-percent}\%) & \UseMacro{res-apache-commons-pool-phase-analysis} (\UseMacro{res-apache-commons-pool-phase-analysis-percent}\%) & \UseMacro{res-apache-commons-pool-phase-execution-collection} (\UseMacro{res-apache-commons-pool-phase-execution-collection-percent}\%) & \UseMacro{res-apache-commons-pool-phase-report} (\UseMacro{res-apache-commons-pool-phase-report-percent}\%)\\
\UseMacro{res-alibaba-fastjson-name} & \UseMacro{res-alibaba-fastjson-ekstazi-selected-rate} & \UseMacro{res-alibaba-fastjson-ijacoco-selected-rate} & \UseMacro{res-alibaba-fastjson-phase-compile} (\UseMacro{res-alibaba-fastjson-phase-compile-percent}\%) & \UseMacro{res-alibaba-fastjson-phase-analysis} (\UseMacro{res-alibaba-fastjson-phase-analysis-percent}\%) & \UseMacro{res-alibaba-fastjson-phase-execution-collection} (\UseMacro{res-alibaba-fastjson-phase-execution-collection-percent}\%) & \UseMacro{res-alibaba-fastjson-phase-report} (\UseMacro{res-alibaba-fastjson-phase-report-percent}\%)\\
\UseMacro{res-finmath-finmath-lib-name} & \UseMacro{res-finmath-finmath-lib-ekstazi-selected-rate} & \UseMacro{res-finmath-finmath-lib-ijacoco-selected-rate} & \UseMacro{res-finmath-finmath-lib-phase-compile} (\UseMacro{res-finmath-finmath-lib-phase-compile-percent}\%) & \UseMacro{res-finmath-finmath-lib-phase-analysis} (\UseMacro{res-finmath-finmath-lib-phase-analysis-percent}\%) & \UseMacro{res-finmath-finmath-lib-phase-execution-collection} (\UseMacro{res-finmath-finmath-lib-phase-execution-collection-percent}\%) & \UseMacro{res-finmath-finmath-lib-phase-report} (\UseMacro{res-finmath-finmath-lib-phase-report-percent}\%)\\
\UseMacro{res-sonyxperiadev-gerrit-events-name} & \UseMacro{res-sonyxperiadev-gerrit-events-ekstazi-selected-rate} & \UseMacro{res-sonyxperiadev-gerrit-events-ijacoco-selected-rate} & \UseMacro{res-sonyxperiadev-gerrit-events-phase-compile} (\UseMacro{res-sonyxperiadev-gerrit-events-phase-compile-percent}\%) & \UseMacro{res-sonyxperiadev-gerrit-events-phase-analysis} (\UseMacro{res-sonyxperiadev-gerrit-events-phase-analysis-percent}\%) & \UseMacro{res-sonyxperiadev-gerrit-events-phase-execution-collection} (\UseMacro{res-sonyxperiadev-gerrit-events-phase-execution-collection-percent}\%) & \UseMacro{res-sonyxperiadev-gerrit-events-phase-report} (\UseMacro{res-sonyxperiadev-gerrit-events-phase-report-percent}\%)\\
\UseMacro{res-brettwooldridge-HikariCP-name} & \UseMacro{res-brettwooldridge-HikariCP-ekstazi-selected-rate} & \UseMacro{res-brettwooldridge-HikariCP-ijacoco-selected-rate} & \UseMacro{res-brettwooldridge-HikariCP-phase-compile} (\UseMacro{res-brettwooldridge-HikariCP-phase-compile-percent}\%) & \UseMacro{res-brettwooldridge-HikariCP-phase-analysis} (\UseMacro{res-brettwooldridge-HikariCP-phase-analysis-percent}\%) & \UseMacro{res-brettwooldridge-HikariCP-phase-execution-collection} (\UseMacro{res-brettwooldridge-HikariCP-phase-execution-collection-percent}\%) & \UseMacro{res-brettwooldridge-HikariCP-phase-report} (\UseMacro{res-brettwooldridge-HikariCP-phase-report-percent}\%)\\
\UseMacro{res-lmdbjava-lmdbjava-name} & \UseMacro{res-lmdbjava-lmdbjava-ekstazi-selected-rate} & \UseMacro{res-lmdbjava-lmdbjava-ijacoco-selected-rate} & \UseMacro{res-lmdbjava-lmdbjava-phase-compile} (\UseMacro{res-lmdbjava-lmdbjava-phase-compile-percent}\%) & \UseMacro{res-lmdbjava-lmdbjava-phase-analysis} (\UseMacro{res-lmdbjava-lmdbjava-phase-analysis-percent}\%) & \UseMacro{res-lmdbjava-lmdbjava-phase-execution-collection} (\UseMacro{res-lmdbjava-lmdbjava-phase-execution-collection-percent}\%) & \UseMacro{res-lmdbjava-lmdbjava-phase-report} (\UseMacro{res-lmdbjava-lmdbjava-phase-report-percent}\%)\\
\UseMacro{res-logic-ng-LogicNG-name} & \UseMacro{res-logic-ng-LogicNG-ekstazi-selected-rate} & \UseMacro{res-logic-ng-LogicNG-ijacoco-selected-rate} & \UseMacro{res-logic-ng-LogicNG-phase-compile} (\UseMacro{res-logic-ng-LogicNG-phase-compile-percent}\%) & \UseMacro{res-logic-ng-LogicNG-phase-analysis} (\UseMacro{res-logic-ng-LogicNG-phase-analysis-percent}\%) & \UseMacro{res-logic-ng-LogicNG-phase-execution-collection} (\UseMacro{res-logic-ng-LogicNG-phase-execution-collection-percent}\%) & \UseMacro{res-logic-ng-LogicNG-phase-report} (\UseMacro{res-logic-ng-LogicNG-phase-report-percent}\%)\\
\UseMacro{res-davidmoten-rxjava-extras-name} & \UseMacro{res-davidmoten-rxjava-extras-ekstazi-selected-rate} & \UseMacro{res-davidmoten-rxjava-extras-ijacoco-selected-rate} & \UseMacro{res-davidmoten-rxjava-extras-phase-compile} (\UseMacro{res-davidmoten-rxjava-extras-phase-compile-percent}\%) & \UseMacro{res-davidmoten-rxjava-extras-phase-analysis} (\UseMacro{res-davidmoten-rxjava-extras-phase-analysis-percent}\%) & \UseMacro{res-davidmoten-rxjava-extras-phase-execution-collection} (\UseMacro{res-davidmoten-rxjava-extras-phase-execution-collection-percent}\%) & \UseMacro{res-davidmoten-rxjava-extras-phase-report} (\UseMacro{res-davidmoten-rxjava-extras-phase-report-percent}\%)\\
\UseMacro{res-bullhorn-sdk-rest-name} & \UseMacro{res-bullhorn-sdk-rest-ekstazi-selected-rate} & \UseMacro{res-bullhorn-sdk-rest-ijacoco-selected-rate} & \UseMacro{res-bullhorn-sdk-rest-phase-compile} (\UseMacro{res-bullhorn-sdk-rest-phase-compile-percent}\%) & \UseMacro{res-bullhorn-sdk-rest-phase-analysis} (\UseMacro{res-bullhorn-sdk-rest-phase-analysis-percent}\%) & \UseMacro{res-bullhorn-sdk-rest-phase-execution-collection} (\UseMacro{res-bullhorn-sdk-rest-phase-execution-collection-percent}\%) & \UseMacro{res-bullhorn-sdk-rest-phase-report} (\UseMacro{res-bullhorn-sdk-rest-phase-report-percent}\%)\\
\UseMacro{res-tabulapdf-tabula-java-name} & \UseMacro{res-tabulapdf-tabula-java-ekstazi-selected-rate} & \UseMacro{res-tabulapdf-tabula-java-ijacoco-selected-rate} & \UseMacro{res-tabulapdf-tabula-java-phase-compile} (\UseMacro{res-tabulapdf-tabula-java-phase-compile-percent}\%) & \UseMacro{res-tabulapdf-tabula-java-phase-analysis} (\UseMacro{res-tabulapdf-tabula-java-phase-analysis-percent}\%) & \UseMacro{res-tabulapdf-tabula-java-phase-execution-collection} (\UseMacro{res-tabulapdf-tabula-java-phase-execution-collection-percent}\%) & \UseMacro{res-tabulapdf-tabula-java-phase-report} (\UseMacro{res-tabulapdf-tabula-java-phase-report-percent}\%)\\
\midrule
\multicolumn{1}{c|}{\textbf{\UseMacro{TH-avg}}} & \UseMacro{res-ekstazi-selected-test-rate-mean} & \UseMacro{res-ijacoco-selected-test-rate-mean} & \UseMacro{res-phase-avg-compile} (\UseMacro{res-phase-avg-compile-percent}\%) & \UseMacro{res-phase-avg-analysis} (\UseMacro{res-phase-avg-analysis-percent}\%) & \UseMacro{res-phase-avg-execution-collection} (\UseMacro{res-phase-avg-execution-collection-percent}\%) & \UseMacro{res-phase-avg-report} (\UseMacro{res-phase-avg-report-percent}\%) \\ 
\bottomrule\end{tabular}

==> tables/table-results-selected-test.tex <==
%% Automatically generated by: results.py table_results_selected_test

\begin{tabular}{l|r|r}
\toprule
\multicolumn{1}{c|}{\multirow{2}{*}{\textbf{\UseMacro{TH-project}}}} & \multicolumn{2}{c}{\textbf{\UseMacro{TH-selected-test-ratio}}} \\
 & \multicolumn{1}{c|}{\ekstazi} & \multicolumn{1}{c}{\ijacocoTool}\\ 
\midrule
\UseMacro{res-asterisk-java-asterisk-java-name} & \UseMacro{res-asterisk-java-asterisk-java-ekstazi-selected-rate} & \UseMacro{res-asterisk-java-asterisk-java-ijacoco-selected-rate}\\
\UseMacro{res-apache-commons-beanutils-name} & \UseMacro{res-apache-commons-beanutils-ekstazi-selected-rate} & \UseMacro{res-apache-commons-beanutils-ijacoco-selected-rate}\\
\UseMacro{res-apache-commons-codec-name} & \UseMacro{res-apache-commons-codec-ekstazi-selected-rate} & \UseMacro{res-apache-commons-codec-ijacoco-selected-rate}\\
\UseMacro{res-apache-commons-collections-name} & \UseMacro{res-apache-commons-collections-ekstazi-selected-rate} & \UseMacro{res-apache-commons-collections-ijacoco-selected-rate}\\
\UseMacro{res-apache-commons-compress-name} & \UseMacro{res-apache-commons-compress-ekstazi-selected-rate} & \UseMacro{res-apache-commons-compress-ijacoco-selected-rate}\\
\UseMacro{res-apache-commons-configuration-name} & \UseMacro{res-apache-commons-configuration-ekstazi-selected-rate} & \UseMacro{res-apache-commons-configuration-ijacoco-selected-rate}\\
\UseMacro{res-apache-commons-dbcp-name} & \UseMacro{res-apache-commons-dbcp-ekstazi-selected-rate} & \UseMacro{res-apache-commons-dbcp-ijacoco-selected-rate}\\
\UseMacro{res-apache-commons-imaging-name} & \UseMacro{res-apache-commons-imaging-ekstazi-selected-rate} & \UseMacro{res-apache-commons-imaging-ijacoco-selected-rate}\\
\UseMacro{res-apache-commons-io-name} & \UseMacro{res-apache-commons-io-ekstazi-selected-rate} & \UseMacro{res-apache-commons-io-ijacoco-selected-rate}\\
\UseMacro{res-apache-commons-lang-name} & \UseMacro{res-apache-commons-lang-ekstazi-selected-rate} & \UseMacro{res-apache-commons-lang-ijacoco-selected-rate}\\
\UseMacro{res-apache-commons-math-name} & \UseMacro{res-apache-commons-math-ekstazi-selected-rate} & \UseMacro{res-apache-commons-math-ijacoco-selected-rate}\\
\UseMacro{res-apache-commons-net-name} & \UseMacro{res-apache-commons-net-ekstazi-selected-rate} & \UseMacro{res-apache-commons-net-ijacoco-selected-rate}\\
\UseMacro{res-apache-commons-pool-name} & \UseMacro{res-apache-commons-pool-ekstazi-selected-rate} & \UseMacro{res-apache-commons-pool-ijacoco-selected-rate}\\
\UseMacro{res-alibaba-fastjson-name} & \UseMacro{res-alibaba-fastjson-ekstazi-selected-rate} & \UseMacro{res-alibaba-fastjson-ijacoco-selected-rate}\\
\UseMacro{res-finmath-finmath-lib-name} & \UseMacro{res-finmath-finmath-lib-ekstazi-selected-rate} & \UseMacro{res-finmath-finmath-lib-ijacoco-selected-rate}\\
\UseMacro{res-sonyxperiadev-gerrit-events-name} & \UseMacro{res-sonyxperiadev-gerrit-events-ekstazi-selected-rate} & \UseMacro{res-sonyxperiadev-gerrit-events-ijacoco-selected-rate}\\
\UseMacro{res-brettwooldridge-HikariCP-name} & \UseMacro{res-brettwooldridge-HikariCP-ekstazi-selected-rate} & \UseMacro{res-brettwooldridge-HikariCP-ijacoco-selected-rate}\\
\UseMacro{res-lmdbjava-lmdbjava-name} & \UseMacro{res-lmdbjava-lmdbjava-ekstazi-selected-rate} & \UseMacro{res-lmdbjava-lmdbjava-ijacoco-selected-rate}\\
\UseMacro{res-logic-ng-LogicNG-name} & \UseMacro{res-logic-ng-LogicNG-ekstazi-selected-rate} & \UseMacro{res-logic-ng-LogicNG-ijacoco-selected-rate}\\
\UseMacro{res-davidmoten-rxjava-extras-name} & \UseMacro{res-davidmoten-rxjava-extras-ekstazi-selected-rate} & \UseMacro{res-davidmoten-rxjava-extras-ijacoco-selected-rate}\\
\UseMacro{res-bullhorn-sdk-rest-name} & \UseMacro{res-bullhorn-sdk-rest-ekstazi-selected-rate} & \UseMacro{res-bullhorn-sdk-rest-ijacoco-selected-rate}\\
\UseMacro{res-tabulapdf-tabula-java-name} & \UseMacro{res-tabulapdf-tabula-java-ekstazi-selected-rate} & \UseMacro{res-tabulapdf-tabula-java-ijacoco-selected-rate}\\
\midrule
\multicolumn{1}{c|}{\textbf{\UseMacro{TH-avg}}} & \UseMacro{res-ekstazi-selected-test-rate-mean} & \UseMacro{res-ijacoco-selected-test-rate-mean} \\ 
\bottomrule\end{tabular}

==> tables/table-results.tex <==
%% Automatically generated by: results.py table_results

\begin{tabular}{lrrr}\toprule Project & $T_i$ & $T_b$ & $T_b / T_i$ \\ \midrule
\UseMacro{res-asterisk-java-asterisk-java-name} & \UseMacro{res-asterisk-java-asterisk-java-ijacoco-time} & \UseMacro{res-asterisk-java-asterisk-java-bjacoco-time} & \UseMacro{res-asterisk-java-asterisk-java-ibjacoco-speedup-time}\\
\UseMacro{res-apache-commons-beanutils-name} & \UseMacro{res-apache-commons-beanutils-ijacoco-time} & \UseMacro{res-apache-commons-beanutils-bjacoco-time} & \UseMacro{res-apache-commons-beanutils-ibjacoco-speedup-time}\\
\UseMacro{res-apache-commons-codec-name} & \UseMacro{res-apache-commons-codec-ijacoco-time} & \UseMacro{res-apache-commons-codec-bjacoco-time} & \UseMacro{res-apache-commons-codec-ibjacoco-speedup-time}\\
\UseMacro{res-apache-commons-collections-name} & \UseMacro{res-apache-commons-collections-ijacoco-time} & \UseMacro{res-apache-commons-collections-bjacoco-time} & \UseMacro{res-apache-commons-collections-ibjacoco-speedup-time}\\
\UseMacro{res-apache-commons-compress-name} & \UseMacro{res-apache-commons-compress-ijacoco-time} & \UseMacro{res-apache-commons-compress-bjacoco-time} & \UseMacro{res-apache-commons-compress-ibjacoco-speedup-time}\\
\UseMacro{res-apache-commons-configuration-name} & \UseMacro{res-apache-commons-configuration-ijacoco-time} & \UseMacro{res-apache-commons-configuration-bjacoco-time} & \UseMacro{res-apache-commons-configuration-ibjacoco-speedup-time}\\
\UseMacro{res-apache-commons-dbcp-name} & \UseMacro{res-apache-commons-dbcp-ijacoco-time} & \UseMacro{res-apache-commons-dbcp-bjacoco-time} & \UseMacro{res-apache-commons-dbcp-ibjacoco-speedup-time}\\
\UseMacro{res-apache-commons-imaging-name} & \UseMacro{res-apache-commons-imaging-ijacoco-time} & \UseMacro{res-apache-commons-imaging-bjacoco-time} & \UseMacro{res-apache-commons-imaging-ibjacoco-speedup-time}\\
\UseMacro{res-apache-commons-io-name} & \UseMacro{res-apache-commons-io-ijacoco-time} & \UseMacro{res-apache-commons-io-bjacoco-time} & \UseMacro{res-apache-commons-io-ibjacoco-speedup-time}\\
\UseMacro{res-apache-commons-lang-name} & \UseMacro{res-apache-commons-lang-ijacoco-time} & \UseMacro{res-apache-commons-lang-bjacoco-time} & \UseMacro{res-apache-commons-lang-ibjacoco-speedup-time}\\
\UseMacro{res-apache-commons-math-name} & \UseMacro{res-apache-commons-math-ijacoco-time} & \UseMacro{res-apache-commons-math-bjacoco-time} & \UseMacro{res-apache-commons-math-ibjacoco-speedup-time}\\
\UseMacro{res-apache-commons-net-name} & \UseMacro{res-apache-commons-net-ijacoco-time} & \UseMacro{res-apache-commons-net-bjacoco-time} & \UseMacro{res-apache-commons-net-ibjacoco-speedup-time}\\
\UseMacro{res-apache-commons-pool-name} & \UseMacro{res-apache-commons-pool-ijacoco-time} & \UseMacro{res-apache-commons-pool-bjacoco-time} & \UseMacro{res-apache-commons-pool-ibjacoco-speedup-time}\\
\UseMacro{res-alibaba-fastjson-name} & \UseMacro{res-alibaba-fastjson-ijacoco-time} & \UseMacro{res-alibaba-fastjson-bjacoco-time} & \UseMacro{res-alibaba-fastjson-ibjacoco-speedup-time}\\
\UseMacro{res-finmath-finmath-lib-name} & \UseMacro{res-finmath-finmath-lib-ijacoco-time} & \UseMacro{res-finmath-finmath-lib-bjacoco-time} & \UseMacro{res-finmath-finmath-lib-ibjacoco-speedup-time}\\
\UseMacro{res-sonyxperiadev-gerrit-events-name} & \UseMacro{res-sonyxperiadev-gerrit-events-ijacoco-time} & \UseMacro{res-sonyxperiadev-gerrit-events-bjacoco-time} & \UseMacro{res-sonyxperiadev-gerrit-events-ibjacoco-speedup-time}\\
\UseMacro{res-brettwooldridge-HikariCP-name} & \UseMacro{res-brettwooldridge-HikariCP-ijacoco-time} & \UseMacro{res-brettwooldridge-HikariCP-bjacoco-time} & \UseMacro{res-brettwooldridge-HikariCP-ibjacoco-speedup-time}\\
\UseMacro{res-lmdbjava-lmdbjava-name} & \UseMacro{res-lmdbjava-lmdbjava-ijacoco-time} & \UseMacro{res-lmdbjava-lmdbjava-bjacoco-time} & \UseMacro{res-lmdbjava-lmdbjava-ibjacoco-speedup-time}\\
\UseMacro{res-logic-ng-LogicNG-name} & \UseMacro{res-logic-ng-LogicNG-ijacoco-time} & \UseMacro{res-logic-ng-LogicNG-bjacoco-time} & \UseMacro{res-logic-ng-LogicNG-ibjacoco-speedup-time}\\
\UseMacro{res-davidmoten-rxjava-extras-name} & \UseMacro{res-davidmoten-rxjava-extras-ijacoco-time} & \UseMacro{res-davidmoten-rxjava-extras-bjacoco-time} & \UseMacro{res-davidmoten-rxjava-extras-ibjacoco-speedup-time}\\
\UseMacro{res-bullhorn-sdk-rest-name} & \UseMacro{res-bullhorn-sdk-rest-ijacoco-time} & \UseMacro{res-bullhorn-sdk-rest-bjacoco-time} & \UseMacro{res-bullhorn-sdk-rest-ibjacoco-speedup-time}\\
\UseMacro{res-tabulapdf-tabula-java-name} & \UseMacro{res-tabulapdf-tabula-java-ijacoco-time} & \UseMacro{res-tabulapdf-tabula-java-bjacoco-time} & \UseMacro{res-tabulapdf-tabula-java-ibjacoco-speedup-time}\\
\bottomrule\end{tabular}
